Lyapunov-Based Reinforcement Learning State Estimator

In this paper, we consider the state estimation problem for nonlinear stochastic discrete-time systems. We combine Lyapunov's method in control theory and deep reinforcement learning to design the state estimator. We theoretically prove the convergence of the bounded estimate error solely using the data simulated from the model. An actor-critic reinforcement learning algorithm is proposed to learn the state estimator approximated by a deep neural network. The convergence of the algorithm is analysed. The proposed Lyapunov-based reinforcement learning state estimator is compared with a number of existing nonlinear filtering methods through Monte Carlo simulations, showing its advantage in terms of estimate convergence even under some system uncertainties such as covariance shift in system noise and randomly missing measurements. To the best of our knowledge, this is the first reinforcement learning based nonlinear state estimator with bounded estimate error performance guarantee.

==> References.tex <==
% Encoding: UTF-8
@article{zhang2020model-2,
	title={Model-Reference Reinforcement Learning for Collision-Free Tracking Control of Autonomous Surface Vehicles},
	author={Zhang, Qingrui and Pan, Wei and Reppa, Vasso},
	journal={arXiv preprint arXiv:2008.07240},
	year={2020}
}

@article{liu2019particle,
	title={Particle filtering with soft state constraints for target tracking},
	author={Liu, Cunjia and Li, Baibing and Chen, Wen-Hua},
	journal={IEEE Transactions on Aerospace and Electronic Systems},
	volume={55},
	number={6},
	pages={3492--3504},
	year={2019},
	publisher={IEEE}
}

@article{li2003survey,
	title={Survey of maneuvering target tracking. Part I. Dynamic models},
	author={Li, X Rong and Jilkov, Vesselin P},
	journal={IEEE Transactions on aerospace and electronic systems},
	volume={39},
	number={4},
	pages={1333--1364},
	year={2003},
	publisher={IEEE}
}

@inproceedings{yadaiah2006neural,
	title={Neural network based state estimation of dynamical systems},
	author={Yadaiah, Narri and Sowmya, G},
	booktitle={The 2006 IEEE International Joint Conference on Neural Network Proceedings},
	pages={1042--1049},
	year={2006},
	organization={IEEE}
}

@article{wilson2009neural,
	title={A neural implementation of the Kalman filter},
	author={Wilson, Robert and Finkel, Leif},
	journal={Advances in neural information processing systems},
	volume={22},
	pages={2062--2070},
	year={2009}
}

@article{krishnan2015deep,
	title={Deep kalman filters},
	author={Krishnan, Rahul G and Shalit, Uri and Sontag, David},
	journal={arXiv preprint arXiv:1511.05121},
	year={2015}
}

@article{zhang2020model-1,
	title={Model-Reference Reinforcement Learning Control of Autonomous Surface Vehicles with Uncertainties},
	author={Zhang, Qingrui and Pan, Wei and Reppa, Vasso},
	journal={arXiv preprint arXiv:2003.13839},
	year={2020}
}

@article{jiang2015global,
	title={Global adaptive dynamic programming for continuous-time nonlinear systems},
	author={Jiang, Yu and Jiang, Zhong-Ping},
	journal={IEEE Transactions on Automatic Control},
	volume={60},
	number={11},
	pages={2917--2929},
	year={2015},
	publisher={IEEE}
}

@incollection{murray2003adaptive,
	title={The adaptive dynamic programming theorem},
	author={Murray, John J and Cox, Chadwick J and Saeks, Richard E},
	booktitle={Stability and control of dynamical systems with applications},
	pages={379--394},
	year={2003},
	publisher={Springer}
}

@article{wang2009adaptive,
	title={Adaptive dynamic programming: An introduction},
	author={Wang, Fei-Yue and Zhang, Huaguang and Liu, Derong},
	journal={IEEE Computational Intelligence Magazine},
	volume={4},
	number={2},
	pages={39--47},
	year={2009},
	publisher={IEEE}
}

@book{nocedal2006numerical,
	title={Numerical optimization},
	author={Nocedal, Jorge and Wright, Stephen},
	year={2006},
	publisher={Springer Science \& Business Media}
}

@book{bertsekas2014constrained,
	title={Constrained optimization and Lagrange multiplier methods},
	author={Bertsekas, Dimitri P},
	year={2014},
	publisher={Academic press}
}

@article{mnih2015human,
	title={Human-level control through deep reinforcement learning},
	author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Rusu, Andrei A and Veness, Joel and Bellemare, Marc G and Graves, Alex and Riedmiller, Martin and Fidjeland, Andreas K and Ostrovski, Georg and others},
	journal={Nature},
	volume={518},
	number={7540},
	pages={529--533},
	year={2015},
	publisher={Nature Publishing Group}
}

@article{deptula2018approximate,
	title={Approximate dynamic programming: Combining regional and local state following approximations},
	author={Deptula, Patryk and Rosenfeld, Joel A and Kamalapurkar, Rushikesh and Dixon, Warren E},
	journal={IEEE Transactions on Neural Networks and Learning Systems},
	volume={29},
	number={6},
	pages={2154--2166},
	year={2018},
	publisher={IEEE}
}

@article{balakrishnan2008issues,
	title={Issues on stability of {ADP} feedback controllers for dynamical systems},
	author={Balakrishnan, SN and Ding, Jie and Lewis, Frank L},
	journal={IEEE Transactions on Systems, Man, and Cybernetics, Part B (Cybernetics)},
	volume={38},
	number={4},
	pages={913--917},
	year={2008},
	publisher={IEEE}
}

@inproceedings{shih2007near,
	title={Near optimal output-feedback control of nonlinear discrete-time systems in nonstrict feedback form with application to engines},
	author={Shih, Peter and Kaul, B and Jagannathan, Sarangapani and Drallmeier, J},
	booktitle={2007 International Joint Conference on Neural Networks},
	pages={396--401},
	year={2007},
	organization={IEEE}
}

@article{abu2005nearly,
	title={Nearly optimal control laws for nonlinear systems with saturating actuators using a neural network HJB approach},
	author={Abu-Khalaf, Murad and Lewis, Frank L},
	journal={Automatica},
	volume={41},
	number={5},
	pages={779--791},
	year={2005},
	publisher={Elsevier}
}

@article{bhandari2018finite,
	title={A finite time analysis of temporal difference learning with linear function approximation},
	author={Bhandari, Jalaj and Russo, Daniel and Singal, Raghav},
	journal={arXiv preprint arXiv:1806.02450},
	year={2018}
}

@inproceedings{kolter2019learning,
	title={Learning Stable Deep Dynamics Models},
	author={Kolter, J Zico and Manek, Gaurav},
	booktitle={Advances in Neural Information Processing Systems},
	pages={11126--11134},
	year={2019}
}

@inproceedings{saunders2018trial,
	title={Trial without error: Towards safe reinforcement learning via human intervention},
	author={Saunders, William and Sastry, Girish and Stuhlmueller, Andreas and Evans, Owain},
	booktitle={Proceedings of the 17th International Conference on Autonomous Agents and MultiAgent Systems},
	pages={2067--2069},
	year={2018},
	organization={International Foundation for Autonomous Agents and Multiagent Systems}
}

@article{fu1970learning,
	title={Learning control systems--Review and outlook},
	author={Fu, King-Sun},
	journal={IEEE Transactions on Automatic Control},
	volume={15},
	number={2},
	pages={210--221},
	year={1970},
	publisher={IEEE}
}

@article{fu1971learning,
	title={Learning control systems and intelligent control systems: An intersection of artifical intelligence and automatic control},
	author={Fu, King-Sun},
	journal={IEEE Transactions on Automatic Control},
	volume={16},
	number={1},
	pages={70--72},
	year={1971},
	publisher={IEEE}
}

@article{antsaklis1990neural,
	title={Neural networks for control systems},
	author={Antsaklis, Panos J},
	journal={IEEE Transactions on Neural Networks},
	volume={1},
	number={2},
	pages={242--244},
	year={1990},
	publisher={IEEE}
}
@book{altman1999constrained,
	title={Constrained Markov decision processes},
	author={Altman, Eitan},
	volume={7},
	year={1999},
	publisher={CRC Press}
}
@book{meyn2012markov,
	title={Markov chains and stochastic stability},
	author={Meyn, Sean P and Tweedie, Richard L},
	year={2012},
	publisher={Springer Science \& Business Media}
}
@techreport{kushner1971introduction,
	title={Introduction to stochastic control},
	author={Kushner, Harold},
	year={1971},
	institution={BROWN UNIV PROVIDENCE RI DIV OF APPLIED MATHEMATICS}
}
@article{howard1960dynamic,
	title={Dynamic programming and {M}arkov processes.},
	author={Howard, Ronald A},
	year={1960},
	publisher={John Wiley}
}
@book{zhou1996robust,
	title={Robust and optimal control},
	author={Zhou, Kemin and Doyle, John Comstock and Glover, Keith and others},
	volume={40},
	year={1996},
	publisher={Prentice hall New Jersey}
}
@misc{baselines,
	author = {Dhariwal, Prafulla and Hesse, Christopher and Klimov, Oleg and Nichol, Alex and Plappert, Matthias and Radford, Alec and Schulman, John and Sidor, Szymon and Wu, Yuhuai and Zhokhov, Peter},
	title = {OpenAI Baselines},
	year = {2017},
	publisher = {GitHub},
	journal = {GitHub repository},
	howpublished = {\url{https://github.com/openai/baselines}},
}

@article{bucsoniu2018reinforcement,
	title={Reinforcement learning for control: Performance, stability, and deep approximators},
	author={Bu{\c{s}}oniu, Lucian and de Bruin, Tim and Toli{\'c}, Domagoj and Kober, Jens and Palunko, Ivana},
	journal={Annual Reviews in Control},
	year={2018},
	publisher={Elsevier}
}

@article{sootla2013toggling,
	title={Toggling a genetic switch using reinforcement learning},
	author={Sootla, Aivar and Strelkowa, Natalja and Ernst, Damien and Barahona, Mauricio and Stan, Guy-Bart},
	journal={arXiv preprint arXiv:1303.3183},
	year={2013}
}
@article{strelkowa2010switchable,
	title={Switchable genetic oscillator operating in quasi-stable mode},
	author={Strelkowa, Natalja and Barahona, Mauricio},
	journal={Journal of The Royal Society Interface},
	volume={7},
	number={48},
	pages={1071--1082},
	year={2010},
	publisher={The Royal Society}
}

@book{sutton2018reinforcement,
	title={Reinforcement learning: An introduction},
	author={Sutton, Richard S and Barto, Andrew G},
	year={2018},
	publisher={MIT press}
}

@article{zhang2012network,
	title={Network-induced constraints in networked control systems—A survey},
	author={Zhang, Lixian and Gao, Huijun and Kaynak, Okyay},
	journal={IEEE Transactions on Industrial Informatics},
	volume={9},
	number={1},
	pages={403--416},
	year={2012},
	publisher={IEEE}
}
@article{lillicrap2015continuous,
	title={Continuous control with deep reinforcement learning},
	author={Lillicrap, Timothy P and Hunt, Jonathan J and Pritzel, Alexander and Heess, Nicolas and Erez, Tom and Tassa, Yuval and Silver, David and Wierstra, Daan},
	journal={arXiv preprint arXiv:1509.02971},
	year={2015}
}

@article{shen2008nonlinear,
	title={On Nonlinear ${H}_\infty$ Filtering for Discrete-Time Stochastic Systems With Missing Measurements},
	author={Shen, Bo and Wang, Zidong and Shu, Huisheng and Wei, Guoliang},
	journal={IEEE Transactions on Automatic Control},
	volume={53},
	number={9},
	pages={2170--2180},
	year={2008},
	publisher={IEEE}
}

@article{wang2012h,
	title={${H}_\infty$ filtering with randomly occurring sensor saturations and missing measurements},
	author={Wang, Zidong and Shen, Bo and Liu, Xiaohui},
	journal={Automatica},
	volume={48},
	number={3},
	pages={556--562},
	year={2012},
	publisher={Elsevier}
}

@article{sinopoli2004kalman,
	title={Kalman filtering with intermittent observations},
	author={Sinopoli, Bruno and Schenato, Luca and Franceschetti, Massimo and Poolla, Kameshwar and Jordan, Michael I and Sastry, Shankar S},
	journal={IEEE Transactions on Automatic Control},
	volume={49},
	number={9},
	pages={1453--1464},
	year={2004},
	publisher={IEEE}
}

@inproceedings{achiam2017constrained,
	title={Constrained policy optimization},
	author={Achiam, Joshua and Held, David and Tamar, Aviv and Abbeel, Pieter},
	booktitle={Proceedings of the 34th International Conference on Machine Learning-Volume 70},
	pages={22--31},
	year={2017},
	organization={JMLR. org}
}

@inproceedings{ammar2015safe,
	title={Safe policy search for lifelong reinforcement learning with sublinear regret},
	author={Ammar, Haitham Bou and Tutunov, Rasul and Eaton, Eric},
	booktitle={International Conference on Machine Learning},
	pages={2361--2369},
	year={2015}
}


@article{smirnova2019distributionally,
	title={Distributionally Robust Reinforcement Learning},
	author={Smirnova, Elena and Dohmatob, Elvis and Mary, J{\'e}r{\'e}mie},
	journal={arXiv preprint arXiv:1902.08708},
	year={2019}
}
@inproceedings{alshiekh2018safe,
	title={Safe reinforcement learning via shielding},
	author={Alshiekh, Mohammed and Bloem, Roderick and Ehlers, R{\"u}diger and K{\"o}nighofer, Bettina and Niekum, Scott and Topcu, Ufuk},
	booktitle={Thirty-Second AAAI Conference on Artificial Intelligence},
	year={2018}
}
@article{cheng2019end,
	title={End-to-End Safe Reinforcement Learning through Barrier Functions for Safety-Critical Continuous Control Tasks},
	author={Cheng, Richard and Orosz, G{\'a}bor and Murray, Richard M and Burdick, Joel W},
	journal={arXiv preprint arXiv:1903.08792},
	year={2019}
}
@inproceedings{haarnoja2017reinforcement,
	title={Reinforcement learning with deep energy-based policies},
	author={Haarnoja, Tuomas and Tang, Haoran and Abbeel, Pieter and Levine, Sergey},
	booktitle={Proceedings of the 34th International Conference on Machine Learning-Volume 70},
	pages={1352--1361},
	year={2017},
	organization={JMLR. org}
}


@inproceedings{haarnoja2018composable,
	title={Composable deep reinforcement learning for robotic manipulation},
	author={Haarnoja, Tuomas and Pong, Vitchyr and Zhou, Aurick and Dalal, Murtaza and Abbeel, Pieter and Levine, Sergey},
	booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
	pages={6244--6251},
	year={2018},
	organization={IEEE}
}


@article{xu2018algorithmic,
	title={Algorithmic Framework for Model-based Reinforcement Learning with Theoretical Guarantees},
	author={Xu, Huazhe and Li, Yuanzhi and Tian, Yuandong and Darrell, Trevor and Ma, Tengyu},
	journal={ICLR},
	year={2019}
}

@inproceedings{deisenroth2011pilco,
	title={PILCO: A model-based and data-efficient approach to policy search},
	author={Deisenroth, Marc and Rasmussen, Carl E},
	booktitle={Proceedings of the 28th International Conference on machine learning (ICML-11)},
	pages={465--472},
	year={2011}
}


@inproceedings{noroozi2008generation,
	title={Generation of \protect{Lyapunov} functions by neural networks},
	author={Noroozi, Navid and Karimaghaee, Paknoosh and Safaei, Fatemeh and Javadi, Hamed},
	booktitle={Proceedings of the World Congress on Engineering},
	volume={2008},
	year={2008}
}
@inproceedings{prokhorov1994lyapunov,
	title={A \protect{Lyapunov} machine for stability analysis of nonlinear systems},
	author={Prokhorov, Danil V},
	booktitle={Proceedings of 1994 IEEE International Conference on Neural Networks (ICNN'94)},
	volume={2},
	pages={1028--1031},
	year={1994},
	organization={IEEE}
}
@inproceedings{serpen2005empirical,
	title={Empirical approximation for \protect{Lyapunov} functions with artificial neural nets},
	author={Serpen, Gursel},
	booktitle={Proceedings. 2005 IEEE International Joint Conference on Neural Networks, 2005.},
	volume={2},
	pages={735--740},
	year={2005},
	organization={IEEE}
}
@inproceedings{prokhorov1999application,
	title={Application of SVM to \protect{Lyapunov} function approximation},
	author={Prokhorov, Danil V and Feldkamp, Lee A},
	booktitle={IJCNN'99. International Joint Conference on Neural Networks. Proceedings (Cat. No. 99CH36339)},
	volume={1},
	pages={383--387},
	year={1999},
	organization={IEEE}
}
@inproceedings{richards2018lyapunov,
	title={The \protect{Lyapunov} Neural Network: Adaptive Stability Certification for Safe Learning of Dynamical Systems},
	author={Richards, Spencer M and Berkenkamp, Felix and Krause, Andreas},
	booktitle={Conference on Robot Learning},
	pages={466--476},
	year={2018}
}
@inproceedings{sootla2013periodic,
	title={On periodic reference tracking using batch-mode reinforcement learning with application to gene regulatory network control},
	author={Sootla, Aivar and Strelkowa, Natalja and Ernst, Damien and Barahona, Mauricio and Stan, Guy-Bart},
	booktitle={52nd IEEE Conference on Decision and Control},
	pages={4086--4091},
	year={2013},
	organization={IEEE}
}


@article{han2019hinf,
	title={\protect{$H_\infty$} Model-free Reinforcement Learning with Robust Stability Guarantee},
	author={Han, Minghao and Tian, Yuan and Zhang, Lixian and Wang, Jun and Pan, Wei},
	journal={NeurIPS 2019 Workshop on Robot Learning: Control and Interaction in the Real World},
	year={2019}
}


@book{anderson2012optimal,
	title={Optimal filtering},
	author={Anderson, Brian DO and Moore, John B},
	year={2012},
	publisher={Courier Corporation}
}

@book{thrun2005probabilistic,
	title={Probabilistic robotics},
	author={Thrun, Sebastian and Burgard, Wolfram and Fox, Dieter},
	year={2005},
	publisher={MIT press Cambridge}
}

@book{bar2004estimation,
	title={Estimation with applications to tracking and navigation: theory algorithms and software},
	author={Bar-Shalom, Yaakov and Li, X Rong and Kirubarajan, Thiagalingam},
	year={2004},
	publisher={John Wiley \& Sons}
}

@inproceedings{duan2016benchmarking,
	title={Benchmarking deep reinforcement learning for continuous control},
	author={Duan, Yan and Chen, Xi and Houthooft, Rein and Schulman, John and Abbeel, Pieter},
	booktitle={International Conference on Machine Learning},
	pages={1329--1338},
	year={2016}
}

@article{zhang2020model,
	title={Model-Reference Reinforcement Learning Control of Autonomous Surface Vehicles with Uncertainties},
	author={Zhang, Qingrui and Pan, Wei and Reppa, Vasso},
	journal={arXiv preprint arXiv:2003.13839},
	year={2020}
}



@article{boutayeb1997convergence,
	title={Convergence analysis of the extended Kalman filter used as an observer for nonlinear deterministic discrete-time systems},
	author={Boutayeb, M and Rafaralahy, H and Darouach, M},
	journal={IEEE Transactions on Automatic Control},
	volume={42},
	number={4},
	pages={581--586},
	year={1997},
	publisher={IEEE}
}

@article{crisan2002survey,
	title={A survey of convergence results on particle filtering methods for practitioners},
	author={Crisan, Dan and Doucet, Arnaud},
	journal={IEEE Transactions on Signal Processing},
	volume={50},
	number={3},
	pages={736--746},
	year={2002},
	publisher={IEEE}
}

@article{doucet2000sequential,
	title={On sequential Monte Carlo sampling methods for Bayesian filtering},
	author={Doucet, Arnaud and Godsill, Simon and Andrieu, Christophe},
	journal={Statistics and Computing},
	volume={10},
	number={3},
	pages={197--208},
	year={2000},
	publisher={Springer}
}

@article{li2012stochastic,
	title={Stochastic stability of the unscented Kalman filter with intermittent observations},
	author={Li, Li and Xia, Yuanqing},
	journal={Automatica},
	volume={48},
	number={5},
	pages={978--981},
	year={2012},
	publisher={Elsevier}
}

@article{xiong2006performance,
	title={Performance evaluation of UKF-based nonlinear filtering},
	author={Xiong, Kai and Zhang, HY and Chan, CW},
	journal={Automatica},
	volume={42},
	number={2},
	pages={261--270},
	year={2006},
	publisher={Elsevier}
}

@article{arulampalam2002tutorial,
	title={A tutorial on particle filters for online nonlinear/non-Gaussian Bayesian tracking},
	author={Arulampalam, M Sanjeev and Maskell, Simon and Gordon, Neil and Clapp, Tim},
	journal={IEEE Transactions on Signal Processing},
	volume={50},
	number={2},
	pages={174--188},
	year={2002},
	publisher={IEEE}
}


@article{kalman1960new,
	title={A new approach to linear filtering and prediction problems},
	author={Kalman, Rudolph Emil},
	journal={Transactions of the ASME -- Journal of Basic Engineering},
	volume={82},
	pages={35--45},
	year={1960}
}

@inproceedings{berkenkamp2017safe,
	title={Safe model-based reinforcement learning with stability guarantees},
	author={Berkenkamp, Felix and Turchetta, Matteo and Schoellig, Angela and Krause, Andreas},
	booktitle={Advances in Neural Information Processing Systems},
	pages={908--918},
	year={2017}
}

@inproceedings{chow2018lyapunov,
	title={A lyapunov-based approach to safe reinforcement learning},
	author={Chow, Yinlam and Nachum, Ofir and Duenez-Guzman, Edgar and Ghavamzadeh, Mohammad},
	booktitle={Advances in Neural Information Processing Systems},
	pages={8092--8101},
	year={2018}
}

@article{chow2019lyapunov,
	title={Lyapunov-based safe policy optimization for continuous control},
	author={Chow, Yinlam and Nachum, Ofir and Faust, Aleksandra and Duenez-Guzman, Edgar and Ghavamzadeh, Mohammad},
	journal={arXiv preprint arXiv:1901.10031},
	year={2019}
}

@inproceedings{chang2019neural,
	title={Neural lyapunov control},
	author={Chang, Ya-Chien and Roohi, Nima and Gao, Sicun},
	booktitle={Advances in Neural Information Processing Systems},
	pages={3245--3254},
	year={2019}
}

@article{han2020actor,
	title={Actor-Critic Reinforcement Learning for Control with Stability Guarantee},
	author={Han, Minghao and Zhang, Lixian and Wang, Jun and Pan, Wei},
	journal={arXiv preprint arXiv:2004.14288},
	year={2020}
}

@article{morimoto2007reinforcement,
	title={Reinforcement learning state estimator},
	author={Morimoto, Jun and Doya, Kenji},
	journal={Neural Computation},
	volume={19},
	number={3},
	pages={730--756},
	year={2007},
	publisher={MIT Press}
}

@article{deisenroth2011robust,
	title={Robust filtering and smoothing with Gaussian processes},
	author={Deisenroth, Marc Peter and Turner, Ryan Darby and Huber, Marco F and Hanebeck, Uwe D and Rasmussen, Carl Edward},
	journal={IEEE Transactions on Automatic Control},
	volume={57},
	number={7},
	pages={1865--1871},
	year={2011},
	publisher={IEEE}
}

@inproceedings{deisenroth2009analytic,
	title={Analytic moment-based Gaussian process filtering},
	author={Deisenroth, Marc Peter and Huber, Marco F and Hanebeck, Uwe D},
	booktitle={Proceedings of the 26th Annual International Conference on Machine Learning},
	pages={225--232},
	year={2009}
}

@article{tsiamis2019sample,
	title={Sample complexity of kalman filtering for unknown systems},
	author={Tsiamis, Anastasios and Matni, Nikolai and Pappas, George J},
	journal={arXiv preprint arXiv:1912.12309},
	year={2019}
}

@article{julier2004unscented,
	title={Unscented filtering and nonlinear estimation},
	author={Julier, Simon J and Uhlmann, Jeffrey K},
	journal={Proceedings of the IEEE},
	volume={92},
	number={3},
	pages={401--422},
	year={2004},
	publisher={IEEE}
}

@book{lewis2017optimal,
	title={Optimal and robust estimation: with an introduction to stochastic control theory},
	author={Lewis, Frank L and Xie, Lihua and Popa, Dan},
	year={2017},
	publisher={CRC press}
}

@book{sarkka2013bayesian,
	title={Bayesian filtering and smoothing},
	author={S{\"a}rkk{\"a}, Simo},
	year={2013},
	publisher={Cambridge University Press}
}

@article{reif1999stochastic,
	title={Stochastic stability of the discrete-time extended Kalman filter},
	author={Reif, Konrad and Gunther, Stefan and Yaz, Engin and Unbehauen, Rolf},
	journal={IEEE Transactions on Automatic Control},
	volume={44},
	number={4},
	pages={714--728},
	year={1999},
	publisher={IEEE}
}


@inproceedings{Tan1993CML,
	title={Multiagent reinforcement learning: Independent vs. cooperative agents},
	author={Ming Tan},
	booktitle={Proceedings of the 10th International Conference on Machine Learning},
	pages={330-337},
	year={1993},
	month={May},
	organization={},
	address =	 {},
	doi={}
}


@inproceedings{Dayan1993NIPS,
	title={Feudal Reinforcement Learning},
	author={Peter Dayan and Geoffrey E. Hinton},
	booktitle={Proceedings of the Advances in Neural Information Processing Systems 5 (NIPS 1992)},
	pages={271--278},
	year={1993},
	month={May},
	organization={},
	address =	 {},
	doi={}
}

@inproceedings{Littman1994ICML,
	title={Markov games as a framework for multi-agent reinforcement learning},
	author={Michael L. Littman},
	booktitle={Proceedings of the 11th International Conference on Machine Learning},
	pages={157-163},
	year={1994},
	month={Jul.},
	organization={},
	address =	 {New Brunswick, NJ, USA},
	doi={10.1016/B978-1-55860-335-6.50027-1}
}


@inproceedings{Agogino2006AAAI,
	title={QUICR-learning for multi-agent coordination},
	author={Adrian K. Agogino and Kagan Tumer},
	booktitle={Proceedings of the 21st national conference on Artificial intelligence - Volume 2},
	pages={1438 -- 1443},
	year={2006},
	month={Jul.},
	organization={},
	address =	 {Boston, Massachusetts},
	doi={10.1145/1160633.1160776}
}

@inproceedings{Panait2006AAMAS,
	title={Lenient Learners in Cooperative Multiagent Systems},
	author={Liviu Panait and Keith Sullivan and Sean Luke},
	booktitle={Proceedings of the 5th International Joint Conference on Autonomous Agents and Multiagent Systems},
	pages={801--803 },
	year={2006},
	month={May},
	organization={},
	address =	 {Hakodate, JapanA},
	doi={10.1145/1160633.1160776}
}

@inproceedings{Soltan2009ACC,
	title={State-dependent trajectory planning and tracking control of unmanned surface vessels},
	author={Reza A. Soltan and Hashem Ashrafiuon and Kenneth R. Muske},
	booktitle={Proceedings of 2009 American Control Conference},
	pages={},
	year={2009},
	month={Jun.},
	organization={IEEE},
	address =	 {St. Louis, MO, USA},
	doi={10.1109/ACC.2009.5160010}
}


@inproceedings{Laetitia2007IROS,
	title={Hysteretic Q-learning : an algorithm for Decentralized Reinforcement Learning in Cooperative Multi-Agent Teams},
	author={La\"etitia Matignon and Guillaume J. Laurent and Nadine Le Fort-Piat},
	booktitle={Proceedings of 2007 IEEE/RSJ International Conference on Intelligent Robots and Systems},
	pages={},
	year={2007},
	month={Dec.},
	organization={IEEE},
	address =	 {San Diego, CA, USA},
	doi={10.1109/IROS.2007.4399095}
}

@inproceedings{Liu2008CDC,
	title={Adaptive robust control of a class of uncertain nonlinear systems with unknown sinusoidal disturbances},
	author={Xiangbin Liu and Hongye Su and Bin Yao and Jian Chu},
	booktitle={Proceedings of 2008 47th IEEE Conference on Decision and Control},
	pages={},
	year={2008},
	month={Dec.},
	organization={IEEE},
	address =	 {Cancun, Mexico, USA},
	doi={10.1109/CDC.2008.4739272}
}


@inproceedings{Berg2008ICRA,
	title={Reciprocal Velocity Obstacles for Real-Time Multi-Agent Navigation},
	author={Jur van den Berg and Ming C. Lin and Dinesh Manocha},
	booktitle={Proceedings of the IEEE International Conference on Robotics and Automation (ICRA)},
	pages={},
	year={2008},
	month={May},
	organization={IEEE},
	address =	 {Pasadena, CA, USA},
	doi={10.1109/ROBOT.2008.4543489}
}


@inproceedings{Greytak2009CDC,
	title={Motion Planning with an Analytic Risk Cost for Holonomic Vehicles},
	author={Matthew Greytak and Franz Hover},
	booktitle={Proceedings of the 48th IEEE Conference on Decision and Control (CDC)},
	pages={},
	year={2009},
	month={Dec.},
	organization={IEEE},
	address =	 {Shanghai, P.R. China},
	doi={10.1109/CDC.2009.5399943}
}


@inproceedings{Fuchs2010CDC,
	title={Cooperative defense within a single-pursuer, two-evader pursuit evasion differential game},
	author={Zachariah E. Fuchs and Pramod P. Khargonekar and Johnny Evers},
	booktitle={Proceedings of the 49th IEEE Conference on Decision and Control (CDC)},
	pages={},
	year={2010},
	month={Dec.},
	organization={IEEE},
	address =	 {Atlanta, GA, USA},
	doi={10.1109/CDC.2010.5717894}
}

@inproceedings{Natarajan2010ICMLA,
	title={Multi-Agent Inverse Reinforcement Learning},
	author={Sriraam Natarajan and Gautam Kunapuli and Kshitij Judah and Prasad Tadepalli and Kristian Kersting and Jude Shavlik},
	booktitle={Proceedings of the 9th International Conference on Machine Learning and Applications},
	pages={},
	year={2010},
	month={Dec.},
	organization={IEEE},
	address =	 {Washington, DC, USA},
	doi={10.1109/ICMLA.2010.65}
}

@inproceedings{Torrey2010AAAI,
	title={Crowd Simulation Via Multi-Agent Reinforcement Learning},
	author={Lisa Torrey},
	booktitle={Proceedings of the 6th AAAI Conference on Artificial Intelligence and Interactive Digital Entertainment},
	pages={89--94},
	year={2010},
	month={Oct.},
	organization={},
	address =	 {Stanford, California, USA },
	doi={}
}

@inproceedings{Vrancx2011ICAART,
	title={Transfer Learning for Multi-agent Coordination},
	author={Peter Vrancx, Yann-Micha\"el De Hauwere, Ann Now\'e},
	booktitle={Proceedings of the 3rd International Conference on Agents and Artificial Intelligence},
	pages={28--30},
	year={2011},
	month={Jan.},
	organization={},
	address =	 {Rome, Italy},
	doi={}
}

@inproceedings{Zhang2011ICAMS,
	title={Transfer Learning in Multi-Agent Reinforcement Learning Domains},
	author={Georgios Boutsioukis and Ioannis Partalas and Ioannis Vlahavas},
	booktitle={Proceedings of the European Workshop on Reinforcement Learning (EWRL 2011)},
	pages={249--260},
	year={2011},
	month={May},
	organization={Springer},
	address =	 {},
	doi={10.1007/978-3-642-29946-9_25}
}

@inproceedings{Lau2012AAMAS,
	title={Coordination guided reinforcement learning},
	author={Qiangfeng Peter Lau and Mong Li Lee and Wynne Hsu},
	booktitle={Proceedings of the 11th International Conference on Autonomous Agents and Multiagent Systems - Volume 1 (AAMAS 2012 )},
	pages={215--222},
	year={2012},
	month={May},
	organization={},
	address =	 {Valencia, Spain},
	doi={}
}


@inproceedings{Hausler2012IFAC,
	title={Cooperative Motion Planning for Multiple Autonomous Marine Vehicles},
	author={Andreas J. H\"{a}usler and Alessandro Saccon and A. Pedro Aguiar and John Hauser and Ant\'{o}nio M. Pascoal},
	booktitle={Proceedings of the IFAC Proceedings Volumes},
	pages={244 -- 249},
	year={2012},
	vol = {45},
	num = {27},
	month={},
	organization={},
	address =	 {Arenzano},
	doi={10.3182/20120919-3-IT-2046.00042}
}

@inproceedings{Zhang2013ICAMS,
	title={Coordinating multi-agent reinforcement learning with limited communication},
	author={Chongjie Zhang and Victor Lesser},
	booktitle={Proceedings of the 2013 International Conference on Autonomous Agents and Multi-agent Systems},
	pages={1101--1108},
	year={2013},
	month={May},
	organization={},
	address =	 {St. Paul, MN, USA },
	doi={}
}


@inproceedings{Amat2013MSDM,
	title={Bayesian Reinforcement Learning for Multiagent Systems with State Uncertainty},
	author={Christopher Amato and Frans A. Oliehoek},
	booktitle={Proceedings of The 8th Annual Workshop on Multiagent Sequential Decision-Making Under Uncertainty (MSDM-2013)},
	pages={},
	year={2013},
	month={May},
	organization={},
	address =	 {St. Paul, Minnesota, USA},
	doi={}
}

@inproceedings{Dahl2013ICASSP,
	title={Improving deep neural networks for LVCSR using rectified linear units and dropout},
	author={George E. Dahl and Tara N. Sainath and Geoffrey E. Hinton},
	booktitle={Proceedings of 2013 IEEE International Conference on Acoustics, Speech and Signal Processing},
	pages={},
	year={2013},
	month={May},
	organization={},
	address =	 {Vancouver, BC, Canada},
	doi={10.1109/ICASSP.2013.6639346}
}


@inproceedings{Zheng2014IFAC,
	title={Trajectory tracking of autonomous vessels using model predictive control},
	author={Huarong Zheng and Rudy R.Negenborn and Gabriel Lodewijks},
	booktitle={Proceedings of the 19th IFAC World Congress},
	pages={},
	volume ={47},
	number = {3},
	year={2014},
	month={May},
	organization={},
	address =	 {Cape Town, South Africa},
	doi={10.3182/20140824-6-ZA-1003.00767}
}

@inproceedings{Holmesparker2014WIC_ACM_IAT,
	title={CLEAN Rewards to Improve Coordination by Removing Exploratory Action Noise},
	author={Chris Holmesparker and Mathew E. Taylor and Adrian K. Agogino and Kagan Tumer},
	booktitle={Proceedings of 2014 IEEE/WIC/ACM International Joint Conferences on Web Intelligence (WI) and Intelligent Agent Technologies (IAT)},
	pages={},
	year={2014},
	month={Aug.},
	organization={},
	address =	 {Warsaw, Poland, USA},
	doi={10.1109/WI-IAT.2014.159}
}

@inproceedings{Schulman2015TRPO,
	title={Trust Region Policy Optimization},
	author={John Schulman and Sergey Levine and Pieter Abbeel and Michael Jordan and Philipp Moritz},
	booktitle={Proceedings of the 31 st International Conference on Machine Learning},
	pages={1889--1897},
	year={2015},
	month={Jun.},
	organization={},
	address =	 {Lille, France},
	doi={}
}

@inproceedings{Kingma2014Adam,
	title={Adam: A Method for Stochastic Optimization},
	author={Diederik P. Kingma and Jimmy Ba},
	booktitle={Proceedings of the 3rd International Conference for Learning Representations (ICLR 2015)},
	pages={},
	year={2015},
	month={May},
	organization={},
	address ={San Diego, USA},
	doi={}
}


@inproceedings{Sukhbaatar2016NIPS,
	title={Learning Multiagent Communication with Backpropagation},
	author={Sainbayar Sukhbaatar and Arthur Szlam and Rob Fergus},
	booktitle={Proceedings of the 30th Conference on Neural Information Processing Systems (NIPS 2016)},
	pages={2252--2260},
	year={2016},
	month={Dec.},
	organization={},
	address =	 {Barcelona, Spain},
	doi={}
}


@inproceedings{Amir2016IJCAI,
	title={Interactive teaching strategies for agent training},
	author={Ofra Amir	and Ece Kamar and Andrey Kolobov and Barbara J. Grosz},
	booktitle={Proceedings of the 25th International Joint Conference on Artificial Intelligence},
	pages={804--811},
	year={2016},
	month={Jul.},
	organization={},
	address =	 {New York, New York, USA },
	doi={}
}


@inproceedings{Klima2016NIPS,
	title={Markov Security Games : Learning in Spatial Security Problems},
	author={Richard Klima and Karl Tuyls and Frans A. Oliehoek},
	booktitle={Proceedings of the 30th Conference on Neural Information Processing Systems (NIPS 2016)},
	pages={},
	year={2016},
	month={Dec.},
	organization={},
	address =	 {Barcelona, Spain},
	doi={}
}


@inproceedings{Chen2016ICRA,
	title={Decentralized non-communicating multiagent collision avoidance with deep reinforcement learning},
	author={Yu Fan Chen and Miao Liu and Michael Everett and Jonathan P. How},
	booktitle={Proceedings of 2017 IEEE International Conference on Robotics and Automation},
	pages={},
	year={2017},
	month={Jun.},
	organization={},
	address =	 {Singapore, Singapore},
	doi={10.1109/ICRA.2017.7989037}
}

@inproceedings{Yin2017KnowledgeTF,
	title={Knowledge Transfer for Deep Reinforcement Learning with Hierarchical Experience Replay},
	author={Haiyan Yin and Sinno Jialin Pan},
	booktitle={Proceedings of the 31st AAAI Conference on Artificial Intelligence},
	page={1640--1646},
	year={2017},
	month={Feb.},
	address={San Francisco, California, USA}
}

@inproceedings{Gupta2017AAMAS,
	title={Cooperative Multi-Agent Control Using Deep Reinforcement Learning},
	author={Jayesh K. Gupta and Maxim Egorov and Mykel Kochenderfer},
	booktitle={Proceedings of the 2017 International Conference on Autonomous Agents and Multiagent Systems (AAMAS 2017)},
	pages={66--83},
	year={2017},
	month={May},
	organization={Springer, Cham},
	address =	 {S\~ao Paulo, Brazil},
	doi={10.1007/978-3-319-71682-4_5}
}

@inproceedings{Silva2017AAMAS,
	title={Simultaneously Learning and Advising in Multiagent Reinforcement Learning},
	author={Felipe Leno da Silva and Ruben Glatt and Anna Helena Reali Costa},
	booktitle={Proceedings of the 16th Conference on Autonomous Agents and Multiagent Systems (AAMAS 2017)},
	pages={1100--1108},
	year={2017},
	month={May},
	organization={Springer, Cham},
	address =	 {S\~ao Paulo, Brazil},
	doi={}
}

@inproceedings{Berkenkamp2017NIPS,
	title={Safe Model-based Reinforcement Learning with Stability Guarantees},
	author={Felix Berkenkamp and Matteo Turchetta and Angela Schoellig and Andreas Krause},
	booktitle={Proceedings of the 31st International Conference on Neural Information Processing Systems (NIPS 2017)},
	pages={},
	year={2017},
	month={Dec.},
	organization={},
	address =	 {Long Beach, CA, USA},
	doi={}
}

@inproceedings{Chen2017IROS,
	title={Socially aware motion planning with deep reinforcement learning},
	author={Yu Fan Chen and Michael Everett and Miao Liu and Jonathan P. How},
	booktitle={Proceedings of 2017 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
	pages={},
	year={2017},
	month={Sep.},
	organization={},
	address =	 {Vancouver, BC, Canada},
	doi={10.1109/IROS.2017.8202312}
}

@inproceedings{Silva2017AAAI,
	title={Accelerating Multiagent Reinforcement Learning through Transfer Learning},
	author={Felipe Leno da Silva and Anna Helena Reali Costa},
	booktitle={Proceedings of the 31st AAAI Conference on Artificial Intelligence (AAAI-17)},
	pages={5034--5035},
	year={2017},
	month={},
	organization={},
	address =	 {},
	doi={}
}

@inproceedings{Haarnoja2018SAC1,
	title={Soft Actor-Critic: Off-Policy Maximum Entropy Deep Reinforcement Learning with a Stochastic Actor},
	author={Tuomas Haarnoja and Aurick Zhou and Pieter Abbeel and Sergey Levine},
	booktitle={Proceedings of the 35th International Conference on Machine Learning (ICML 2018)},
	pages={1861--1870},
	volume={80},
	year={2018},
	month={Jul.},
	organization={},
	address ={Stockholmsm\"{a}ssan, Stockholm Sweden},
	doi={}
}

@inproceedings{Fujimoto2018TD3,
	title={Addressing Function Approximation Error in Actor-Critic Methods},
	author={Scott Fujimoto and Herke van Hoof and David Meger},
	pages={1587--1596},
	volume={80},
	year={2018},
	month={Jul.},
	organization={},
	address ={Stockholmsm\"{a}ssan, Stockholm Sweden},
	doi={}
}


@inproceedings{Li2019AAAI,
	title={Robust Multi-Agent Reinforcement Learning via Minimax Deep Deterministic Policy Grad},
	author={Shihui Li and Yi Wu and Xinyue Cui and Honghua Dong and Fei Fang and Stuart Russell},
	booktitle={Proceedings of the 33rd AAAI Conference on Artificial Intelligence (AAAI-19)},
	pages={},
	year={2019},
	month={Jan.-Feb.},
	organization={},
	address =	 {Honolulu, Hawaii, USA},
	doi={}
}


@inproceedings{Han2019NIPS,
	title={$H_{\infty}$ Model-free Reinforcement Learning with Robust Stability Guarantee},
	author={Minghao Han and Yuan Tian and Lixian Zhang and Jun Wang and Wei Pan},
	booktitle={Proceedings of the 33rd Conference on Neural Information Processing Systems (NeurIPS 2019)},
	pages={},
	year={2019},
	month={Dec.},
	organization={},
	address ={Vancouver, Canada},
	doi={}
}

%------------------------------------------------------------------------------
%   ---------------------------     Articles     ---------------------------
%------------------------------------------------------------------------------

@article{Guan1991TAC,
	title={A novel approach to the design of unknown input observers},
	author={Yuping Guan and Mehrdad Saif},
	journal={IEEE Transactions on Automatic Control},
	volume={36},
	number={5},
	pages={632 -- 635},
	year={1991},
	month={May},
	doi={10.1109/9.76372}
}


@article{Sutton1992CSM,
	title={Reinforcement learning is direct adaptive optimal control},
	author={R.S. Sutton and A.G. Barto and R.J. Williams},
	journal={IEEE Control Systems Magazine },
	volume={12},
	number={2},
	pages={19 -- 22},
	year={1992},
	month={Apr.},
	doi={10.1109/37.126844}
}

@article{Shen1995TAC,
	title={Robust $H_{\infty}$ control of uncertain nonlinear system via state feedback},
	author={T. Shen and K. Tamura},
	journal={IEEE Transactions on Automatic Control},
	volume={40},
	number={4},
	pages={766 -- 768},
	year={1995},
	month={Apr.},
	doi={10.1109/9.376091}
}

@article{Burmeister1997IEE,
	title={Application of multi-agent systems in traffic and transportation},
	author={Birgit Burmeister and Afsaneh Haddadi and Guido Matylis},
	journal={IEE Proceedings - Software Engineering},
	volume={144},
	number={1},
	pages={51--60},
	year={1997},
	month={Feb.},
	doi={10.1049/ip-sen:19971023}
}

@article{Beard1997Auto,
	title={Galerkin approximations of the generalized Hamilton-Jacobi-Bellman equation},
	author={Randal W. Beard and George N. Saridis and John T. Wen},
	journal={Automatica},
	volume={33},
	number={12},
	pages={2159 -- 2177},
	month={},
	year={1997},
	doi ={10.1016/S0005-1098(97)00128-3}
}


@article{Arai2002TransRobAuto,
	title={Editorial: Advances in Multi-Robot Systems},
	author={Tamio Arai and Enrico Pagello and Lynne E. Parker},
	journal={IEEE Transactions on Robotics and Automation},
	volume={18},
	number={5},
	pages={655--661},
	month={Dec.},
	year={2002},
	doi={10.1109/TRA.2002.806024}
}

@article{Guo2000Auto,
	title={Nonlinear decentralized control of large-scale power systems},
	author={Yi Guo and David J. Hill and Youyi Wang},
	journal={Automatica},
	volume={36},
	number={9},
	pages={1275--1289},
	month={Sep.},
	year={2000},
	doi={10.1016/S0005-1098(00)00038-8}
}

@article{Do2006Auto,
	title={Global robust adaptive path following of underactuated ships},
	author={K.D. Do and J. Pan},
	journal={Automatica},
	volume={42},
	number={10},
	pages={1713 -- 1722},
	month={Oct.},
	year={2006},
	doi={10.1016/j.automatica.2006.04.026}
}

@article{Skjetnea2005Auto,
	title={Adaptive maneuvering, with experiments, for a model ship in a marine control laboratory},
	author={Roger Skjetne and Thor I. Fossen and Petar V. Kokotovi\'{c}},
	journal={Mathematics of Operations Research},
	volume={41},
	number={},
	pages={289 -- 298},
	month={},
	year={2005},
	doi ={10.1016/j.automatica.2004.10.006}
}

@article{Bernstein2002MOR,
	title={The Complexity of Decentralized Control of Markov Decision Processes},
	author={Daniel S. Bernstein and Robert Givan and Neil Immerman and Shlomo Zilberstein},
	journal={Mathematics of Operations Research},
	volume={24},
	number={5},
	pages={819 -- 840},
	month={},
	year={2002}
}


@article{Haddad2002IJACSP,
	title={Direct adaptive control for non-linear uncertain systems
		with exogenous disturbances},
	author={Wassim M. Haddad and Tomohisa Hayakawa},
	journal={International Journal of Adaptive Control and Signal Processing},
	volume={16},
	number={2},
	pages={151 -- 172},
	month={Feb.},
	year={2002},
	doi = {10.1002/acs.678}
}



@article{Lafferriere2002SCL,
	title={Decentralized control of vehicle formations},
	author={G. Lafferriere and A. Williams and J. Caughman and J.J.P. Veerman},
	journal={Systems \& Control Letters},
	volume={5},
	number={},
	pages={899 -- 910},
	month={},
	year={2005},
	doi = {10.1016/j.sysconle.2005.02.004}
}


@article{Sola2008TransRob,
	title={Fusing Monocular Information in Multicamera SLAM},
	author={Joan Sola and Andre Monin and Michel Devy and Teresa Vidal-Calleja},
	journal={IEEE Transactions on Robotics},
	volume={24},
	number={5},
	pages={958--968},
	month={Oct.},
	year={2008},
	doi={10.1109/TRO.2008.2004640}
}


@article{Bakule2008ARC,
	title={Decentralized control: An overview},
	author={Lubom\'{i}r Bakule},
	journal={Annual Reviews in Control},
	volume={32},
	number={},
	pages={87--98},
	month={},
	year={2008},
	doi={10.1016/j.arcontrol.2008.03.004}
}

@article{Busoniu2008TSMC,
	title={A Comprehensive Survey of Multiagent Reinforcement Learning},
	author={Lucian Bu\c soniu, Robert Babu\v ska, and Bart De Schutter},
	journal={IEEE Transactions on Systems, Man, and Cybernetics, Part C: Applications and Reviews},
	volume={38},
	number={2},
	pages={156-172},
	year={2008},
	month={Mar.},
	doi={10.1109/TSMCC.2007.913919}
}

@article{Ren2004JGCD,
	Author = {Wei Ren and Randal W. Beard},
	Title = {Decentralized Scheme for Spacecraft Formation Flying via the Virtual Structure Approach},
	Journal = {Journal of Guidance, Control, and Dynamics},
	Volume = {27},
	Number = {1},
	Pages = {706--716},
	Month = {Jan./Feb.},
	Year = {2004},
	doi={10.2514/1.9287}
}

@article{Panait2005AAMAS,
	Title = {Cooperative Multi-Agent Learning: {T}he State of the Art},
	Author = {Liviu Panait and Sean Luke},
	Journal = {Autonomous Agents and Multi-Agent Systems},
	Volume = {11},
	Number = {3},
	Pages = {387--434},
	Month = {Nov.},
	Year = {2005},
	doi={10.1007/s10458-005-2631-2}
}

@article{Do2004Automatica,
	Title = {Robust adaptive path following of underactuated ships},
	Author = {K.D. Do and Z.P. Jiang and J. Pan},
	Journal = {Automatica},
	Volume = {40},
	Number = {6},
	Pages = {929 -- 944},
	Month = {Nov.},
	Year = {2004},
	doi={10.1016/j.automatica.2004.01.021}
} 

@ARTICLE{Olfati-Saber2007IEEE,
	author = {Reza Olfati-Saber and J. Alex Fax and Richard M. Murray},
	title = {Consensus and Cooperation in Networked Multi-Agent Systems},
	journal = {Proceedings of the IEEE},
	month={Mar.},
	year = {2007},
	volume = {95},
	number={1},
	publisher =  {IEEE},
	address =  {New York City, USA},
	page = {1215--233},
	doi={10.1109/JPROC.2006.887293}
}


@ARTICLE{Oliehoek2008JAIR,
	author = {Frans A. Oliehoek and Matthijs T.J. Spaan and Nikos Vlassis},
	title = { Optimal and Approximate Q-value Functions for Decentralized POMDPs},
	journal = {Journal of Artificial Intelligence Research},
	month={Jan.},
	year = {2009},
	volume={32},
	number = {1},
	pages = {289 -- 353},
	doi={}
}


@ARTICLE{Lewis2009CSM,
	author = {Frank L. Lewis and Draguna Vrabie},
	title = {Reinforcement Learning and Adaptive Dynamic Programming for Feedback Control},
	journal = {IEEE Circuits and Systems Magazine},
	month={Jan.},
	year = {2009},
	volume={9},
	number = {3},
	pages = {32--50},
	doi={10.1109/MCAS.2009.933854}
}

@ARTICLE{Verscheure2009TAC,
	author = {Diederik Verscheure and Bram Demeulenaere and Jan Swevers and Joris De Schutter and Moritz Diehl},
	title = {Time-Optimal Path Tracking for Robots: {A} Convex Optimization Approach},
	journal = {IEEE Transactions on Automatic Control},
	month={Sep.},
	year = {2009},
	volume={54},
	number = {10},
	pages = {2318--2327},
	doi={10.1080/00207170902948027}
}



@article{Al-Tamimi2008TSC,
	title = {A Short-Range Ship Navigation System Based on Ladar Imaging and Target Tracking for Improved Safety and Efficiency},
	author = {Asma Al-Tamimi and Frank L. Lewis and Murad Abu-Khalaf},
	journal = {IEEE Transactions on Systems, Man, and Cybernetics, Part B (Cybernetics)},
	volume = {38},
	number = {4},
	pages = {943 -- 949},
	month ={Aug.},
	year = {2008},
	doi = {10.1109/TSMCB.2008.9266148}
}

@article{Ramon2009TITS,
	title = {A Short-Range Ship Navigation System Based on Ladar Imaging and Target Tracking for Improved Safety and Efficiency},
	author = {Antonio Ram\'{O}n and Jimenez Ruiz and Fernando Seco Granja},
	journal = {IEEE Transactions on Intelligent Transportation Systems},
	volume = {10},
	number = {1},
	pages = {186 -- 197},
	month ={Mar.},
	year = {2012},
	doi = {10.1109/TITS.2008.2011698}
}

@ARTICLE{Ren2009IJC,
	author = {Wei Ren},
	title = {Distributed leaderless consensus algorithms for networked {E}uler-{L}agrange systems},
	journal = {International Journal of Control},
	month={Nov.},
	year = {2009},
	volume={82},
	number = {11},
	pages = {2137--2149},
	doi={10.1080/00207170902948027}
}

@ARTICLE{Mayne2000Auto,
	author = {D.Q. Mayne and J.B. Rawlings and C.V. Rao and P.O.M.Scokaert},
	title = {Constrained model predictive control: Stability and optimality},
	journal = {Automatica},
	month={Jun.},
	year = {2000},
	volume={36},
	number = {6},
	pages = {789 -- 814},
	doi={10.1016/S0005-1098(99)00214-9}
}


@article{Matignon2012KNR,
	title={Independent reinforcement learners in cooperative Markov games: A survey regarding coordination problems},
	author={La\"etitia Matignon and Guillaume J. Laurent and Nadine Le Fort-Piat},
	journal={The Knowledge Engineering Review},
	volume={27},
	number={1},
	pages={1--38},
	year={2012},
	doi={10.1016/j.arcontrol.2018.09.005}
}

@article{Melo2011AI,
	title={Decentralized MDPs with sparse interactions},
	author={Francisco S. Melo and Manuela Veloso},
	journal={Artificial Intelligence},
	volume={175},
	number={},
	pages={1757--1789},
	year={2011},
	doi={}
}

@article{Perera2012TITS,
	title = {Maritime Traffic Monitoring Based on Vessel Detection, Tracking, State Estimation, and Trajectory Prediction},
	author = {Lokukaluge P. Perera and Paulo Oliveira and and C. Guedes Soares},
	journal = {IEEE Transactions on Intelligent Transportation Systems},
	volume = {13},
	number = {3},
	pages = {1188 -- 1200},
	month ={Sep.},
	year = {2012},
	doi = {10.1109/TITS.2012.2187282}
}


@article{Tuyls2012AIMag,
	title={Multiagent Learning: Basics, Challenges, and Prospects},
	author={Karl Tuyls and Gerhard Weiss},
	journal={AI Magazine},
	volume={},
	number={},
	pages={41-52},
	year={2012},
	doi={10.1609/aimag.v33i3.2426}
}

@article{Yu2012IET,
	title={Sliding mode tracking control of an underactuated surface vessel},
	author={R. Yu and Q. Zhu and G. Xia and Z. Liu},
	journal={IET Control Theory \& Applications},
	volume={6},
	number={3},
	pages={461 --  466},
	year={2012},
	doi={10.1049/iet-cta.2011.0176}
}


@article{Hover2012IJRR,
	title={Advanced perception, navigation and planning for autonomous in-water ship hull inspection},
	author={Franz S Hover and  Ryan M Eustice and  Ayoung Kim and  Brendan Englot and  Hordur Johannsson and  Michael Kaess and John J. Leonard},
	journal={The International Journal of Robotics Research},
	volume={31},
	number={12},
	pages={1445 -- 1464},
	year={2012},
	doi={10.1177/0278364912461059}
}

@article{Peng2013,
	title={Leaderless and leader-follower cooperative control of multiple marine surface vehicles with unknown dynamics},
	author={Zhouhua Peng and Dan Wang and Tieshan Li and Zhiliang Wu},
	journal={Nonlinear Dynamics},
	volume={74},
	number={},
	pages={95 -- 106},
	year={2013},
	doi={10.1007/s11071-013-0951-3}
}

@article{Kahveci2013Auto,
	title={Adaptive steering control for uncertain ship dynamics and stability analysis},
	author={Nazli E.Kahveci and Petros A. Ioannou},
	journal={Automatica},
	volume={49},
	number={3},
	pages={685--697},
	month={May},
	year={2013},
	doi={10.1016/j.automatica.2012.11.026}
}


@article{Chowdhary2013IJACSP,
	title={Concurrent learning adaptive control of linear systems with exponentially convergent bounds},
	author={Girish Chowdhary and Tansel Yucelen and Maximillian M\"{u}hlegg  and Eric N. Johnson},
	journal={International Journal of Adaptive Control and Signal Processing},
	volume={27},
	number={4},
	pages={280--301},
	month={May},
	year={2013},
	doi={10.1002/acs.2297}
}



@article{Campbel2013ARC,
	title = {A review on improving the autonomy of unmanned surface vehicles through intelligent collision avoidance manoeuvres},
	author = "S. Campbell and W. Naeem and G.W. Irwin",
	journal = "Annual Reviews in Control",
	volume = "36",
	number = "2",
	pages = "267 - 283",
	year = "2012",
	issn = "1367-5788",
	doi = "10.1016/j.arcontrol.2012.09.008"
}

@ARTICLE{Wang2013TCST,
	author = {Jianan Wang and Ming Xin},
	title = {Integrated Optimal Formation Control of Multiple Unmanned Aerial Vehicles},
	journal = {{IEEE} Transactions on Control Systems Technology},
	number = {5},
	volume = {21},
	pages = {1731--1744},
	month={Sep.},
	year = {2013},
	doi={10.1109/TCST.2012.2218815}
}


@ARTICLE{Kober2013IJRR,
	author = {Jens Kober and James Andrew Bagnell and Jan Peters},
	title = {Reinforcement learning in robotics: A survey},
	journal = {International Journal of Robotics Research},
	number = {32},
	volume = {11},
	pages = {1238 -- 1274},
	month={Sep.},
	year = {2013},
	doi={10.1177/0278364913495721}
} 


@article{Mondal2013ISA,
	title={Chattering free adaptive multivariable sliding mode controller for systems with matched and mismatched uncertainty},
	author={Sanjoy Mondal and Chitralekha Mahanta},
	journal={ISA Transactions},
	volume={52},
	number={},
	pages={335 -- 341},
	month={},
	year={2013},
	doi ={10.1016/j.isatra.2012.12.007}
}


@ARTICLE{Sonnenburg2013JFR,
	author = {Christian R. Sonnenburg and Craig A. Woolsey},
	title = {Integrated Optimal Formation Control of Multiple Unmanned Aerial Vehicles},
	journal = {Journal of Field Robotics},
	number = {30},
	volume = {3},
	pages = {371 -- 398},
	month={May/Jun.},
	year = {2013},
	doi={10.1002/rob.21452}
} 

@ARTICLE{Svec2014AR,
	author = {Petr  \v{S}vec and Atul Thakur and Eric Raboin and Brual C. Shah and Satyandra K. Gupta },
	title = {Target following with motion prediction for unmanned surface vehicle operating in cluttered environments},
	journal = {International Journal of Robotics Research},
	number = {36},
	volume = {},
	pages = {383 -- 405},
	month={Apr.},
	year = {2014},
	doi={10.1007/s10514-013-9370-z}
} 




@article{Rezaee2014TIE,
	Author = {Hamed Rezaee and Farzaneh Abdollahi},
	Journal = {{IEEE} Transactions on Industrial Electronics},
	Month = {Jan.},
	Number = {1},
	Pages = {347-354},
	Title = {A Decentralized Cooperative Control Scheme With Obstacle Avoidance for a Team of Mobile Robots},
	Volume = {61},
	Year = {2014},
	doi = {10.1109/TIE.2013.2245612}
}  




@article{Dahmani2014TITS,
	title={Observer-Based Robust Control of Vehicle Dynamics for Rollover Mitigation in Critical Situations},
	author={Hamid Dahmani and Olivier Pag\`{e}s and Ahmed El Hajjaji and Nawal Daraoui},
	journal={{IEEE} Transactions on Intelligent Transportation Systems },
	volume={15},
	number={1},
	pages={274--284},
	month =  {Jan.},
	year={2014},
	doi={110.1109/TITS.2013.2281135}
}


@article{Marinescu2014LDecen_MARL,
	title={Decentralised Multi-Agent Reinforcement Learning for Dynamic and Uncertain Environments},
	author={Andrei Marinescu and Ivana Dusparic and Adam Taylor and Vinny Cahill and Siobh\'an Clarke},
	journal={arXiv preprint arXiv:1409.4561},
	volume={},
	number={},
	pages={},
	year={2014},
	doi={}
}

@article{Lin2014Cmp_MultiSing,
	title={Comparison of Multi-agent and Single-agent Inverse Learning on a Simulated Soccer Example},
	author={Xiaomin Lin and Peter A. Beling and Randy Cogill},
	journal={arXiv preprint arXiv:1403.6822},
	volume={},
	number={},
	pages={},
	year={2014},
	doi={}
}




@ARTICLE{Adamek2015TMech,
	author = {Thomas Adamek and Christopher A. Kitts and Ignacio Mas},
	title = {Gradient-Based Cluster Space Navigation for Autonomous Surface Vessels},
	journal = {IEEE/ASME Transactions on Mechatronics },
	number = {2},
	volume = {20},
	pages = {506--518},
	month={Apr.},
	year = {2015},
	doi={10.1109/TMECH.2013.2297152}
}


@ARTICLE{Mnih2015Nature,
	author = {Volodymyr Mnih and Koray Kavukcuoglu and David Silver and Andrei A. Rusu and Joel Veness and Marc G. Bellemare and Alex Graves and Martin Riedmiller and Andreas K. Fidjeland and Georg Ostrovski and Stig Petersen, Charles Beattie and Amir Sadik and Ioannis Antonoglou and Helen King and Dharshan Kumaran and Daan Wierstra and Shane Legg and Demis Hassabis},
	title = {Human-level control through deep reinforcement learning},
	journal = {Nature},
	month={Feb.},
	year = {2015},
	volume={518},
	number = {},
	pages = {529--533},
	doi={10.1038/nature14236}
}

@article{Li2015TITS,
	title={Extended-State-Observer-Based Double-Loop Integral Sliding-Mode Control of Electronic Throttle Valve},
	author={Yongfu Li and Bin Yang and Taixiong Zheng and Yinguo Li and Mingyue Cui and Srinivas Peeta},
	journal={{IEEE} Transactions on Intelligent Transportation Systems },
	volume={16},
	number={5},
	pages={2501--2510},
	month =  {Mar.},
	year={2015},
	doi={10.1109/TITS.2015.2410282}
}


@article{Tampuu2015CoopComp_DMARL,
	title={Multiagent Cooperation and Competition with Deep Reinforcement Learning},
	author={Ardi Tampuu and Tambet Matiisen and Dorian Kodelja  and Ilya Kuzovkin and Kristjan Korjus and  Juhan Aru and Jaan Aru and Raul Vicente},
	journal={arXiv preprint arXiv:1511.08779},
	volume={},
	number={},
	pages={},
	year={2015},
	doi={}
}

@article{Hao2015TAAS,
	title={Multiagent Reinforcement Social Learning toward Coordination in Cooperative Multiagent Systems},
	author={Jianye Hao and Dongping Huang and Yi Cai and Ho-fung Leung},
	journal={ACM Transactions on Autonomous and Adaptive Systems },
	volume={9},
	number={4},
	pages={20:1--20:20},
	year={2015},
	month={Jan.},
	doi={10.1145/2644819}
}

@article{Bloembergen2015JAI,
	title={Evolutionary Dynamics of Multi-Agent Learning: A Survey},
	author={Daan Bloembergen and Karl Tuyls and Daniel Hennes and Michael Kaisers},
	journal={Journal of Artificial Intelligence Research},
	volume={53},
	number={},
	pages={659--697},
	year={2015},
	doi={10.1016/j.arcontrol.2018.09.005}
}


@article{Jiang2015TAC,
	title={Global Adaptive Dynamic Programming for Continuous-Time Nonlinear Systems},
	author={Yu Jiang and Zhong-Ping Jiang},
	journal={IEEE Transactions on Automatic Control},
	volume={60},
	number={11},
	pages={2917 -- 2929},
	month= {Mar.},
	year={2015},
	doi={10.1109/TAC.2015.2414811}
}

@article{Yu2015TC,
	title={Multiagent Learning of Coordination in Loosely Coupled Multiagent Systemsy},
	author={Chao Yu and Minjie Zhang and Fenghui Ren and Guozhen Tan},
	journal={IEEE Transactions on Cybernetics},
	volume={45},
	number={12},
	pages={2853--2867},
	year={2015},
	month={Jan.},
	doi={10.1109/TCYB.2014.2387277}
}


@article{Lillicrap2015DDPG,
	title={Continuous control with deep reinforcement learning},
	author={Timothy P. Lillicrap and Jonathan J. Hunt and Alexander Pritzel and Nicolas Heess and Tom Erez and Yuval Tassa and David Silver and Daan Wierstra},
	journal={arXiv preprint arXiv:1509.02971},
	year={2015}
}

@article{Hasselt2015DDQN,
	title={Deep Reinforcement Learning with Double Q-learning},
	author={Hado van Hasselt and Arthur Guez and David Silver},
	journal={arXiv preprint arXiv:1509.06461},
	year={2015}
}


@article{Hausknecht2015DRQN,
	title={Deep Recurrent Q-Learning for Partially Observable MDPs},
	author={Matthew Hausknecht and Peter Stone},
	journal={arXiv preprint arXiv:1507.06527},
	volume={},
	number={},
	pages={},
	year={2015},
	doi={}
}

@article{Gonzalez2016TITS,
	title={A Review of Motion Planning Techniques for Automated Vehicles},
	author={David Gonz\'{a}lez and Joshu\'{e} P\'{e}rez and Vicente Milan\'{e}s and Fawzi Nashashibi},
	journal={IEEE Transactions on Intelligent Transportation Systems},
	volume={17},
	number={4},
	pages={1135 -- 1145},
	year={2016},
	doi={10.1109/TITS.2015.2498841}
}


@article{Wang2016TC,
	title={A Novel Extreme Learning Control Framework of Unmanned Surface Vehicles},
	author={Ning Wang and Jing-Chao Sun and Meng Joo Er and Yan-Cheng Liu},
	journal={IEEE Transactions on Cybernetics},
	volume={46},
	number={5},
	pages={1106 -- 1117},
	year={2016},
	month={May},
	doi={10.1109/TCYB.2015.2423635}
}

@article{Vamvoudakis2016TNNLS,
	title={Asymptotically Stable Adaptive?Optimal Control Algorithm With Saturating Actuators and Relaxed Persistence of Excitation},
	author={Kyriakos G. Vamvoudakis and Marcio Fantini Miranda and Jo\~{a}o P. Hespanha},
	journal={IEEE Transactions on Neural Networks and Learning Systems},
	volume={27},
	number={11},
	pages={2386--2398},
	year={2016},
	month={Nov.},
	doi={10.1109/TNNLS.2015.2487972}
}

@article{Shwartz2016RL_AutoDr,
	title={Safe, Multi-Agent, Reinforcement Learning for Autonomous Driving},
	author={Shai Shalev-Shwartz and Shaked Shammah and Amnon Shashua},
	journal={arXiv preprint arXiv:1610.03295},
	year={2016}
}

@article{Foerster2016Learn2Comm,
	title={Learning to Communicate to Solve Riddles with Deep Distributed Recurrent Q-Networks},
	author={Jakob N. Foerster and Yannis M. Assael and Nando de Freitas and Shimon Whiteson},
	journal={arXiv preprint arXiv:1602.02672},
	volume={},
	number={},
	pages={},
	year={2016},
	doi={}
}

@article{Panagou2017TAC,
	title={A Distributed Feedback Motion Planning Protocol for Multiple Unicycle Agents of Different Classes},
	author={Dimitra Panagou},
	journal={IEEE Transactions on Automatic Control},
	volume={62},
	number={3},
	pages={1178 -- 1193},
	month= {Mar.},
	year={2017},
	doi={10.1109/TAC.2016.2576020}
}

@article{Chiang2018RAL,
	title={{COLREG-RRT}: An {RRT}-Based {COLREGS}-Compliant Motion Planner for Surface Vehicle Navigation},
	author={Hao-Tien Lewis Chiang  and Lydia Tapia},
	journal={IEEE Robotics and Automation Letters },
	volume={3},
	number={3},
	pages={2024 -- 2031},
	month= {Jul.},
	year={2018},
	doi={10.1109/LRA.2018.2801881}
}

@article{Parisotto2016Actor-Mimic,
	title={Actor-Mimic: Deep Multitask and Transfer Reinforcement Learning},
	author={Emilio Parisotto and Jimmy Ba and Ruslan Salakhutdin},
	journal={arXiv preprint arXiv:1511.06342},
	volume={},
	number={},
	pages={},
	year={2016},
	doi={}
}

@article{Rusu2016PolicyDistill,
	title={Policy Distillation},
	author={Andrei A. Rusu and Sergio G\'omez Colmenarejo and \c{C} a\v{g}lar G\"ul\c{c}ehre and Guillaume Desjardins and James Kirkpatrick and Razvan Pascanu and Volodymyr Mnih and Koray Kavukcuoglu and Raia Hadsell},
	journal={arXiv preprint arXiv:1511.06295},
	volume={},
	number={},
	pages={},
	year={2016},
	doi={}
}

@article{Rusu2016ProgNN,
	title={Progressive Neural Networks},
	author={Andrei A. Rusu and Neil C. Rabinowitz and Guillaume Desjardins and Hubert Soyer and James Kirkpatrick and Koray Kavukcuoglu and Razvan Pascanu and Raia Hadsell},
	journal={arXiv preprint arXiv:1606.04671},
	volume={},
	number={},
	pages={},
	year={2016},
	doi={}
}

@article{Foerster2016Learn2Comm_DMARL,
	title={Learning to Communicate with Deep Multi-Agent Reinforcement Learning},
	author={Jakob N. Foerster and Yannis M. Assael and Nando de Freitas and Shimon Whiteson},
	journal={arXiv preprint arXiv:1605.06676},
	volume={},
	number={},
	pages={},
	year={2016},
	doi={}
}

@article{He2016Opponent_Model,
	title={Opponent Modeling in Deep Reinforcement Learning},
	author={He He and Jordan Boyd-Graber and Kevin Kwok and Hal Daum\'e III},
	journal={arXiv preprint 	arXiv:1609.05559 },
	volume={},
	number={},
	pages={},
	year={2016},
	doi={}
}

@article{Zhou2016Sparse_Interactiions,
	title={Multi-agent Reinforcement Learning with Sparse Interactions by Negotiation and Knowledge Transfer},
	author={Luowei Zhou and Pei Yang and Chunlin Chen and Yang Gao},
	journal={arXiv preprint arXiv:1508.05328},
	volume={},
	number={},
	pages={},
	year={2016},
	doi={}
}

@article{Lazaridou2016MA_NLP,
	title={Multi-Agent Cooperation and the Emergence of (Natural) Language},
	author={Angeliki Lazaridou and Alexander Peysakhovich and Marco Baroni},
	journal={arXiv preprint arXiv:1612.07182},
	volume={},
	number={},
	pages={},
	year={2016},
	doi={}
}

@article{Menell2016Coop_InvRL,
	title={Cooperative Inverse Reinforcement Learning},
	author={Dylan Hadfield-Menell and Anca Dragan and Pieter Abbeel and Stuart Russell},
	journal={arXiv preprint arXiv:1606.03137},
	volume={},
	number={},
	pages={},
	year={2016},
	doi={}
}


@article{Abdallah2016JMLR,
	title={Addressing Environment Non-Stationarity by Repeating Q-learning Updates},
	author={Sherief Abdallah, Michael Kaisers},
	journal={Journal of Machine Learning Research},
	volume={17},
	number={46},
	pages={1--31},
	year={2016},
	doi={}
}


@article{Kong2017Obj_Searc,
	title={Collaborative Deep Reinforcement Learning for Joint Object Search},
	author={Xiangyu Kong and Bo Xin and Yizhou Wang and Gang Hua},
	journal={arXiv preprint arXiv:1702.05573},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}


@article{Bansal2017Emerg_MA-Comp,
	title={Emergent Complexity via Multi-Agent Competition},
	author={Trapit Bansal and Jakub Pachocki and Szymon Sidor and Ilya Sutskever and Igor Mordatch},
	journal={arXiv preprint arXiv:1710.03748},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}

@article{Chebotarl2017MB_MF,
	title={Combining Model-Based and Model-Free Updates for Trajectory-Centric Reinforcement Learning},
	author={Yevgen Chebotar and Karol Hausman and Marvin Zhang and Gaurav Sukhatme and Stefan Schaal and Sergey Levineh},
	journal={arXiv preprint 	arXiv:1703.03078},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}


@article{Kirkpatrick2017EWC,
	title={Overcoming catastrophic forgetting in neural networks},
	author={James Kirkpatrick and Razvan Pascanu and Neil Rabinowitz, Joel Veness and Guillaume Desjardins and Andrei A. Rusu and Kieran Milan and John Quan and Tiago Ramalho and Agnieszka Grabska-Barwinska and Demis Hassabis and Claudia Clopath and Dharshan Kumaran and Raia Hadsell},
	journal={arXiv preprint arXiv:1612.00796},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}


@article{Bloisi2017TITS,
	title={Enhancing Automatic Maritime Surveillance Systems With Visual Information},
	author={Domenico D. Bloisi and Fabio Previtali and Andrea Pennisi and Daniele Nardi and Michele Fiorini},
	journal={{IEEE} Transactions on Intelligent Transportation Systems },
	volume={18},
	number={4},
	pages={824 -- 833},
	month =  {Apr.},
	year={2017},
	doi={10.1109/TITS.2016.2591321}
}


@article{Mao2017ACCNet,
	title={ACCNet: Actor-Coordinator-Critic Net for ``Learning-to-Communicate" with Deep Multi-agent Reinforcement Learning},
	author={Hangyu Mao and Zhibo Gong and Yan Ni and Xiangyu Liu and Quanbin Wang and Weichen Ke and Chao Ma and Yiping Song and Zhen Xiao},
	journal={arXiv preprint arXiv:1706.03235},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}

@article{Liu2017TIE,
	title={Extended State Observer-Based Sliding-Mode Control for Three-Phase Power Converters},
	author={Jianxing Liu and Sergio Vazquez and Ligang Wu and Abraham Marquez and Huijun Gao and Leopoldo G. Franquelo},
	journal={IEEE Transactions on Industrial Electronics},
	volume={64},
	number={1},
	pages={22--31},
	year={2017},
	doi={10.1109/TIE.2016.2610400}
}


@article{Peng2017BiCNet,
	title={Multiagent Bidirectionally-Coordinated Nets: Emergence of Human-level Coordination in Learning to Play StarCraft Combat Games},
	author={Peng Peng and Ying Wen and Yaodong Yang and Quan Yuan and Zhenkun Tang and Haitao Long and Jun Wang},
	journal={arXiv preprint arXiv:1703.10069 },
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}


@article{Li2017TITS,
	title={Reinforcement Learning-Based Variable Speed Limit Control Strategy to Reduce Traffic Congestion at Freeway Recurrent Bottlenecks},
	author={Zhibin Li and Pan Liu and Chengcheng Xu and Hui Duan and Wei Wang},
	journal={IEEE Transactions on Intelligent Transportation Systems},
	volume={18},
	number={11},
	pages={3204--3217},
	year={2017},
	month={Nov.},
	doi={10.1109/TITS.2017.2687620}
}

@article{Foerster2017Counterfactual,
	title={Counterfactual Multi-Agent Policy Gradients},
	author={Jakob N. Foerster and Gregory Farquhar and Triantafyllos Afouras and Nantas Nardelli and Shimon Whiteson},
	journal={arXiv preprint arXiv:1705.08926},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}

@article{Mordatch2017CompoLangu,
	title={Emergence of Grounded Compositional Language in Multi-Agent Populations},
	author={Igor Mordatch and Pieter Abbeel},
	journal={arXiv preprint 	arXiv:1703.04908},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}

@article{Das2017Coop_Dialog,
	title={Learning Cooperative Visual Dialog Agents with Deep Reinforcement Learning},
	author={Abhishek Das and Satwik Kottur and Jos\'e M. F. Moura and Stefan Lee and Dhruv Batra},
	journal={arXiv preprint arXiv:1703.06585},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}

@article{Shediva2017Adap_Meta,
	title={Continuous Adaptation via Meta-Learning in Nonstationary and Competitive Environments},
	author={Maruan Al-Shedivat and Trapit Bansal and Yuri Burda and Ilya Sutskever and Igor Mordatch and Pieter Abbeel},
	journal={arXiv preprint arXiv:1710.03641},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}

@article{Hwangbo2017RAL,
	title={Control of a Quadrotor With Reinforcement Learning},
	author={Jemin Hwangbo and Inkyu Sa and Roland Siegwart and Marco Hutter},
	journal={IEEE Robotics and Automation Letters},
	volume={2},
	number={4},
	pages={2096 -- 2103},
	month = {Oct.},
	year={2017},
	doi={10.1109/LRA.2017.2720851}
}


@article{Omidshafiei2017Multi-task,
	title={Deep Decentralized Multi-task Multi-Agent Reinforcement Learning under Partial Observability},
	author={Shayegan Omidshafiei and Jason Pazis and Christopher Amato and Jonathan P. How and John Vian},
	journal={arXiv preprint arXiv:1703.06182v4},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}

@article{Rajeswaran2017ICLR,
	title={{EPO}PT: LEARNING ROBUST NEURAL NETWORK POLICIES USING MODEL ENSEMBLES},
	author={Aravind Rajeswaran and Sarvjeet Ghotra and Balaraman Ravindran and Sergey Levine},
	journal={arXiv preprint arXiv:1610.01283},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}

@article{Pinto2017Rob_ARL,
	title={Robust Adversarial Reinforcement Learning},
	author={Lerrel Pinto and James Davidson and Rahul Sukthankar and Abhinav Gupta},
	journal={arXiv preprint arXiv:1703.02702},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}

@article{Havrylov2017Learn2Comm,
	title={Emergence of Language with Multi-agent Games: Learning to Communicate with Sequences of Symbols },
	author={Serhii Havrylov and Ivan Titov},
	journal={arXiv preprint arXiv:1705.11192},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}

@article{Hong2017PolicyInf_MAS,
	title={A Deep Policy Inference Q-Network for Multi-Agent Systems},
	author={Zhang-Wei Hong and Shih-Yang Su and Tzu-Yun Shann and Yi-Hsiang Chang and Chun-Yi Lee},
	journal={arXiv preprint arXiv:1712.07893},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}

@article{Johansen2016TITS,
	title = {Ship Collision Avoidance and COLREGS Compliance Using Simulation-Based Control Behavior Selection With Predictive Hazard Assessment
	},
	author = {Tor Arne Johansen and Tristan Perez  and Andrea Cristofaro},
	journal = {IEEE Transactions on Intelligent Transportation Systems},
	volume = {17},
	number = {2},
	pages = {3407 -- 3422},
	month ={May},
	year = {2016},
	doi = {10.1109/TITS.2016.2551780}
}


@article{Tu2018TITS,
	title = "Exploiting AIS Data for Intelligent Maritime Navigation: A Comprehensive Survey From Data to Methodology",
	author = "Enmei Tu and Guanghao Zhang and Lily Rachmawati and Eshan Rajabally and Guang-Bin Huang
	",
	journal = " IEEE Transactions on Intelligent Transportation Systems ",
	volume = "19",
	number = {5},
	pages = "1559 --1582",
	month ={May},
	year = "2018",
	issn = "",
	doi = "10.1109/TITS.2017.27245514"
}
@article{Haarnoja2018SAC2,
	title={Soft Actor-Critic Algorithms and Applications},
	author={Tuomas Haarnoja and Aurick Zhou, Kristian Hartikainen and George Tucker and Sehoon Ha and Jie Tan and Vikash Kumar and Henry Zhu and Abhishek Gupta and Pieter Abbeel and Sergey Levine},
	journal={arXiv preprint arXiv:1812.05905},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}


@article{Li2019OE,
	title = "Distributed coordination for collision avoidance of multiple ships considering ship maneuverability",
	author = "Shijie Li and Jialun Liu and Rudy R. Negenborn",
	journal = "Ocean Engineering",
	volume = "181",
	pages = "212 - 226",
	year = "2019",
	issn = "0029-8018",
	doi = "10.1016/j.oceaneng.2019.03.054"
	
}

@article{Levander2017IEEE,
	title={Autonomous ships on the high seas},
	author={Oskar Levander},
	journal={IEEE Spectrum},
	volume={54},
	number={2},
	pages={26 -- 31},
	year={2017},
	doi={10.1109/MSPEC.2017.7833502}
}

@article{Berkenkamp2017arXiv,
	title={Safe Model-based Reinforcement Learning with Stability Guarantees},
	author={Felix Berkenkamp and Matteo Turchetta and Angela P. Schoellig and Andreas Krause},
	journal={arXiv preprint 	arXiv:1705.08551},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}


@article{Lanctot2017Unified_GameTheo,
	title={A Unified Game-Theoretic Approach to Multiagent Reinforcement Learning},
	author={Marc Lanctot and Vinicius Zambaldi and Audr\=unas Gruslys and Angeliki Lazaridou and Karl Tuyls and Julien P\'erolat and David Silver and Thore Graepel},
	journal={arXiv preprint arXiv:1711.00832},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}

@article{Wang2017OE,
	title={Finite-time observer based accurate tracking control of a marine vehicle with complex unknowns},
	author={Ning Wang and Shuailin Lv and Weidong Zhang and Zhongzhong Liu and Meng Joo Er},
	journal={arXiv preprint arXiv:1711.00832},
	volume={145},
	number={15},
	pages={406 -- 415},
	year={2017},
	doi={10.1016/j.oceaneng.2017.09.062}
}


@article{Schulman2017PPO,
	title={Proximal policy optimization algorithms},
	author={John Schulman and Filip Wolski and Prafulla Dhariwal and Alec Radford and Oleg Klimov},
	journal={arXiv preprint arXiv:1707.06347},
	year={2017}
}

@article{Kong2017MasterSlave,
	title={Revisiting the Master-Slave Architecture in Multi-Agent Deep Reinforcement Learning},
	author={Xiangyu Kong and Bo Xin and Fangchen Liu and Yizhou Wang},
	journal={arXiv preprint arXiv:1712.07305},
	volume={},
	number={},
	pages={},
	year={2017},
	doi={}
}



@article{Jiang2018ATOC,
	title={Learning Attentional Communication for Multi-Agent Cooperation},
	author={Jiechuan Jiang and Zongqing Lu},
	journal={arXiv preprint arXiv:1805.07733},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}


@article{Chow2018arXiv,
	title={A Lyapunov-based Approach to Safe Reinforcement Learning},
	author={Yinlam Chow and Ofir Nachum and Edgar Duenez-Guzman and Mohammad Ghavamzadeh},
	journal={arXiv preprint arXiv:1805.07708},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}


@article{Foerste2018BAD,
	title={Bayesian Action Decoder for Deep Multi-Agent Reinforcement Learning},
	author={Jakob N. Foerster and Francis Song and Edward Hughes and Neil Burch and Iain Dunning and Shimon Whiteson and Matthew Botvinick and Michael Bowling},
	journal={arXiv preprint arXiv:1811.01458},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}

@article{Zhang2018AST,
	title={Aerodynamic model-based robust adaptive control for close formation flight},
	author={Qingrui Zhang and Hugh H.T. Liu},
	journal={Aerospace Science and Technology},
	volume={79},
	number={},
	pages={5 -- 16},
	year={2018},
	doi={10.1016/j.ast.2018.05.029}
}

@article{Zhu2018IJRNC,
	title={Design and experimental evaluation of robust motion synchronization control for multivehicle system without velocity measurements},
	author={Bo Zhu and Qingrui Zhang and Hugh H.T. Liu},
	journal={International Journal of Robust and Nonlinear Control},
	volume={28},
	number={7},
	pages={5437 -- 5463},
	year={2018},
	doi={10.1002/rnc.4323}
}

@ARTICLE{Zhang2018TIE,
	author = {Qingrui Zhang and Hugh H.T. Liu},
	title = {{UDE}-Based Robust Command Filtered Backstepping Control for Close Formation Flight},
	journal = { IEEE Transactions on Industrial Electronics},
	month={Nov.},
	year = {2018},
	volume = {65},
	pages = {8818-8827},
	number = {11},
	doi={10.1109/TIE.2018.2811367},
	note={}
} 

@article{Kiumarsi2018TNNLS,
	title={Optimal and Autonomous Control Using Reinforcement Learning: A Survey},
	author={Bahare Kiumarsi  and  Kyriakos G. Vamvoudakis and Hamidreza Modares and Frank L. Lewis},
	journal={IEEE Transactions on Neural Networks and Learning Systems},
	volume={29},
	number={6},
	pages={2042 -- 2062},
	year={2018},
	month={Jun.},
	doi={10.1109/TNNLS.2017.2773458}
}


@article{Raileanu2018SOM,
	title={Modeling Others using Oneself in Multi-Agent Reinforcement Learning},
	author={Roberta Raileanu and Emily Denton and Arthur Szlam and Rob Fergus},
	journal={arXiv preprint arXiv:1802.09640},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}


@article{Omidshafiei2018Learn2Teach,
	title={Learning to Teach in Cooperative Multiagent Reinforcement Learning},
	author={Shayegan Omidshafiei and Dong-Ki Kim and Miao Liu and Gerald Tesauro and Matthew Riemer and Christopher Amato and Murray Campbell and Jonathan P. How},
	journal={arXiv preprint 	arXiv:1805.07830},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}


@article{Hoang2018DecenGP_MA,
	title={Collective Online Learning via Decentralized Gaussian Processes in Massive Multi-Agent Systems},
	author={Trong Nghia Hoang and Jonathan How and Quang Minh Hoang and Kian Hsiang Low},
	journal={arXiv preprint arXiv:1805.09266},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}

@article{Le2018Coord_MAIL,
	title={Coordinated Multi-Agent Imitation Learning},
	author={Hoang M. Le and Yisong Yue and Peter Carr and Patrick Lucey},
	journal={arXiv preprint arXiv:1703.03121},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}


@article{Foerster2018OpponentLearn,
	title={Learning with Opponent-Learning Awareness},
	author={Jakob N. Foerster and Richard Y. Chen and Maruan Al-Shedivat and Shimon Whiteson and Pieter Abbeel and Igor Mordatch},
	journal={arXiv preprint arXiv:1709.04326},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}

@article{Haarnoja2018SAC,
	title={Soft Actor-Critic: Off-Policy Maximum Entropy Deep Reinforcement Learning with a Stochastic Actor},
	author={Tuomas Haarnoja and Aurick Zhou and Pieter Abbeel and Sergey Levine},
	journal={arXiv preprint arXiv:1801.01290},
	year={2018}
}

@article{Busoniu2018ARC,
	title={Reinforcement learning for control: Performance, stability, and deep approximators},
	author={Lucian Bu\c oniua and Timde Bruin and Domagoj Toli\'c and Jens Kober and Ivana Palunko},
	journal={Annual Reviews in Control},
	volume={46},
	number={},
	pages={8--28},
	year={2018},
	doi={10.1016/j.arcontrol.2018.09.005}
}

@article{Cao2018EmergComm,
	title={Emergent Communication through Negotiation},
	author={Kris Cao and Angeliki Lazaridou and Marc Lanctot and Joel Z Leibo and Karl Tuyls and Stephen Clark},
	journal={arXiv preprint arXiv:1804.03980},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}


@article{Levine2018RL_Tut&Revi,
	title={Reinforcement Learning and Control as Probabilistic
		Inference: Tutorial and Review},
	author={Sergey Levine},
	journal={arXiv preprint arXiv:1805.00909},
	year={2018}
}

@article{Foerster2018StabExpRep_DMARL,
	title={Stabilising Experience Replay for Deep Multi-Agent Reinforcement Learning},
	author={Jakob Foerster and Nantas Nardelli and Gregory Farquhar and Triantafyllos Afouras and Philip. H. S. Torr and Pushmeet Kohli and Shimon Whiteson},
	journal={arXiv preprint arXiv:1702.08887},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}


@article{Schulman2018HD_GAE,
	title={High-Dimensional Continuous Control Using Generalized Advantage Estimation},
	author={John Schulman and Philipp Moritz and Sergey Levine and Michael Jordan and Pieter Abbeel},
	journal={arXiv preprint arXiv:1506.02438},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}

@article{Yang2018MeanField_DMARL,
	title={Mean Field Multi-Agent Reinforcement Learning},
	author={Yaodong Yang and Rui Luo and Minne Li and Ming Zhou and Weinan Zhang and Jun Wang},
	journal={arXiv preprint arXiv:1802.05438},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}


@article{Lowe2018Coop_Comp,
	title={Multi-Agent Actor-Critic for Mixed Cooperative-Competitive Environments},
	author={Ryan Lowe and Yi Wu and Aviv Tamar and Jean Harb and Pieter Abbeel and Igor Mordatch},
	journal={arXiv preprint arXiv:1706.02275},
	volume={},
	number={},
	pages={},
	year={2018},
	doi={}
}

@article{Lin2018TG,
	title={Multi-agent Inverse Reinforcement Learning for Two-person Zero-sum Games},
	author={Xiaomin Lin and Peter A. Beling and and Randy Cogill},
	journal={IEEE Transactions on Games},
	volume={10},
	number={1},
	pages={56-68},
	year={2018},
	month={Mar.},
	doi={10.1109/TCIAIG.2017.2679115}
}

@article{Palmer2018Lenient,
	title={Lenient Multi-Agent Deep Reinforcement Learning},
	author={Gregory Palmer and Karl Tuyls and Daan Bloembergen and Rahul Savan},
	journal={arXiv preprint arXiv:1707.04402},
	volume={},
	number={},
	pages={},
	year={2018},
	month={},
	doi={}
}



@article{Zhang2018DecMARL,
	title={Fully Decentralized Multi-Agent Reinforcement Learning with Networked Agents},
	author={Kaiqing Zhang and Zhuoran Yang and Han Liu and Tong Zhang and Tamer Ba\c{s}ar},
	journal={arXiv preprint arXiv:1802.08757},
	volume={},
	number={},
	pages={},
	year={2018},
	month={},
	doi={}
}


@article{Grau-Moya2018TwoPlayerGame,
	title={Balancing Two-Player Stochastic Games with Soft Q-Learning},
	author={Jordi Grau-Moya and Felix Leibfried and Haitham Bou-Ammar},
	journal={arXiv preprint arXiv:1802.03216},
	volume={},
	number={},
	pages={},
	year={2018},
	month={},
	doi={}
}

@article{Nguyen2019DMARL_Review,
	title={Deep Reinforcement Learning for Multi-Agent Systems: A Review of Challenges, Solutions and Applications},
	author={Thanh Thi Nguyen and Ngoc Duy Nguyen and Saeid Nahavandi},
	journal={arXiv preprint arXiv:1812.11794},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}

@article{Chow2019arXiv,
	title={Lyapunov-based Safe Policy Optimization for Continuous Control},
	author={Yinlam Chow and Ofir Nachum and Aleksandra Faust and Edgar Duenez-Guzman and Mohammad Ghavamzadeh},
	journal={arXiv preprint 	arXiv:1901.10031},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}

@article{Vasarhelyi2018SR,
	title={Optimized flocking of autonomous drones in confined environments},
	author={G\'{a}bor V\'{a}s\'{a}rhelyi and Csaba Vir\'{a}gh and Gerg\H{o} Somorjai and Tam\'{a}s Nepusz and Agoston E. Eiben and Tam\'{a}s Vicsek},
	journal={Science Robotics},
	volume={3},
	number={20},
	pages={},
	year={2018},
	doi={10.1126/scirobotics.aat3536}
}

@article{McGuire12019SR,
	title={Minimal navigation solution for a swarm of tiny flying robots to explore an unknown environment},
	author={K.N. McGuire1 and C. De Wagter and K. Tuyls and H.J. Kappen and G. C. H. E. de Croon},
	journal={Science Robotics},
	volume={4},
	number={35},
	pages={},
	year={2019},
	doi={10.1126/scirobotics.aaw9710}
}

@article{Iqbal12019ArXiv,
	title={Actor-Attention-Critic for Multi-Agent Reinforcement Learning},
	author={Shariq Iqbal and Fei Sha},
	journal={arXiv preprint arXiv:1810.0291},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}

@article{Abdelaal2018OE,
	title={Nonlinear Model Predictive Control for trajectory tracking and collision avoidance of underactuated vessels with disturbances},
	author={Mohamed Abdelaal and Martin Fr\"{a}nzle and Axel Hahn},
	journal={Ocean Engineering},
	volume={160},
	number={15},
	pages={168 --180},
	month={Jul.},
	year={2018},
	doi={10.1016/j.oceaneng.2018.04.026}
}

@article{Jiang2018arXiv,
	title={Learning attentional communication for multi-agent cooperation},
	author={Jiechuan Jiang and Zongqing Lu},
	journal={arXiv preprint arXiv:1805.07733},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}


@article{Liu2019arXiv_MAGA,
	title={multi-agent game abstraction via graph attention neural network},
	author={Yong Liu and Weixun Wang and Yujing Hu and Jianye Hao and Xingguo Chen and Yang Gao1},
	journal={arXiv preprint arXiv:1911.10715},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}


@article{Qin2019arXiv,
	title={Lyapunov Criterion for Stochastic Systems and Its Applications in Distributed Computation},
	author={Yuzhen Qin and Ming Cao and and Brian D. O. Anderson},
	journal={arXiv preprint 	arXiv:1902.04332},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}






@article{Kim2019Hierarch_Teaching,
	title={Learning Hierarchical Teaching in Cooperative Multiagent Reinforcement Learning},
	author={Dong Ki Kim and Miao Liu and Shayegan Omidshafiei and Sebastian Lopez-Cot and Matthew Riemer and Golnaz Habibi and Gerald Tesauro and Sami Mourad and Murray Campbell and Jonathan P. How},
	journal={arXiv preprint arXiv:1903.03216},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}

@article{Kim2019SchedNet,
	title={Learning to Schedule Communication in Multi-agent Reinforcement Learning},
	author={Daewoo Kim and Sangwoo Moon and David Hostallero and Wan Ju Kang and Taeyoung Lee and Kyunghwan Son and Yung Yi},
	journal={arXiv preprint arXiv:1902.01554},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}


@article{Shen2019ActivePercep,
	title={Active Perception in Adversarial Scenarios using Maximum Entropy Deep Reinforcement Learning},
	author={Macheng Shen and Jonathan P. H},
	journal={arXiv preprint arXiv:1902.05644},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}

@article{Wen2019Recu_Reason,
	title={Probabilistic Recursive Reasoning for Multi-Agent Reinforcement Learning},
	author={Ying Wen and Yaodong Yang and Rui Luo and Jun Wang and Wei Pan},
	journal={arXiv preprint arXiv:1901.09207},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}

@article{Wen2019Gene_Reason,
	title={Multi-Agent Generalized Recursive Reasoning},
	author={Ying Wen and Yaodong Yang and Rui Luo and Jun Wang},
	journal={arXiv preprint arXiv:1901.09216},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}


@article{Menda2019TITS,
	title={Deep Reinforcement Learning for Event-Driven Multi-Agent Decision Processes},
	author={Kunal Menda and Yi-Chun Chen and Justin Grana and James W. Bono and Brendan D. Tracey and Mykel J. Kochenderfer and David Wolpert},
	journal={IEEE Transactions on Intelligent Transportation Systems},
	volume={20},
	number={4},
	pages={1259--1268},
	year={2019},
	doi={10.1109/TITS.2018.2848264}
}


@article{Hu2019TITS,
	title={A Multiobjective Optimization Approach for COLREGs-Compliant Path Planning of Autonomous Surface Vehicles Verified on Networked Bridge Simulators},
	author={Liang Hu and Wasif Naeem and Eshan Rajabally and Graham Watson and Terry Mills and Zakirul Bhuiyan and Craig Raeburn and Ivor Salter and Claire Pekcan},
	journal={IEEE Transactions on Intelligent Transportation Systems},
	volume={21},
	number={3},
	pages={1167--1179},
	year={2019},
	doi={10.1109/TITS.2019.2902927}
}




@article{Jones2019STTE,
	title={Autonomous marine environmental monitoring: Application in decommissioned oil fields},
	author={Daniel O.B.Jones and Andrew R.Gates and Veerle A.I.Huvenne and Alexander B.Phillips and Brian J.Bett},
	journal={Science of The Total Environment},
	volume={668},
	number={10},
	pages={835-- 853},
	year={2019},
	doi={10.1016/j.scitotenv.2019.02.310}
}



@article{Czarnecki2019Distilling,
	title={Distilling Policy Distillation},
	author={Wojciech Marian Czarnecki and Razvan Pascanu and Simon Osindero and Siddhant M. Jayakumar and Grzegorz Swirszcz and Max Jaderberg},
	journal={arXiv preprint arXiv:1902.02186},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}



@article{Lutjens2019SafeRL,
	title={Safe Reinforcement Learning with Model Uncertainty Estimates},
	author={Bj\"orn L\"utjens and Michael Everett and Jonathan P. How},
	journal={arXiv preprint arXiv:1810.08700},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}

@article{Parisotto2019ConcMeta,
	title={Concurrent Meta Reinforcement Learnings},
	author={Emilio Parisotto and Soham Ghosh and Sai Bhargav Yalamanchi and Varsha Chinnaobireddy and Yuhuai Wu and Ruslan Salakhutdinov},
	journal={arXiv preprint arXiv:1903.02710},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}

@article{Vlontzos2019Detect_MARL,
	title={Multiple Landmark Detection using Multi-Agent Reinforcement Learning},
	author={Athanasios Vlontzos and Amir Alansary and Konstantinos Kamnitsas and Daniel Rueckert and Bernhard Kainz},
	journal={arXiv preprint arXiv:1907.00318},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}

@article{Meyer2019arXiv_ASV,
	title={Taming an autonomous surface vehicle for path following and collision avoidance using deep reinforcement learning},
	author={Eivind Meyer and Haakon Robinson and Adil Rasheed and Omer San},
	journal={IEEE Access},
	volume={8},
	number={},
	pages={41466 -- 41481},
	year={2020},
	doi={10.1109/ACCESS.2020.2976586}
}


@article{Zhou2019Access,
	title={Learn to Navigate: Cooperative Path Planning for Unmanned Surface Vehicles Using Deep Reinforcement Learning},
	author={Xinyuan Zhou and Peng Wu and Haifeng Zhang and Weihong Guo  and Yuanchang Liu},
	journal={IEEE Access},
	volume={7},
	number={},
	pages={165262 -- 165278},
	month = {Nov.},
	year={2019},
	doi={10.1109/ACCESS.2019.2953326}
}

@article{Tian2019ROMMEO,
	title={A Regularized Opponent Model with Maximum Entropy Objective},
	author={Zheng Tian and Ying Wen and Zhichen Gong and Faiz Punakkath and Shihao Zou and Jun Wang},
	journal={arXiv preprint arXiv:1905.08087},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}


@article{Wadhwania2019PD-VM_MARL,
	title={Policy Distillation and Value Matching in Multiagent Reinforcement Learning},
	author={Samir Wadhwania and Dong-Ki Kim and Shayegan Omidshafieiy and Jonathan P. How},
	journal={arXiv preprint arXiv:1903.06592},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}


@article{Li2019Logistics,
	title={A Cooperative Multi-Agent Reinforcement Learning Framework for Resource Balancing in Complex Logistics Network},
	author={Xihan Li and Jia Zhang and Jiang Bian and Yunhai Tong and Tie-Yan Liu},
	journal={arXiv preprint arXiv:1903.00714},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}

@article{Qu2019Value_Propag,
	title={Value Propagation for Decentralized Networked Deep Multi-agent Reinforcement Learning},
	author={Chao Qu and Shie Mannor and Huan Xu and Yuan Qi and Le Song and Junwu Xiong},
	journal={arXiv preprint arXiv:1901.09326 },
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}

@article{Everett2019arXiv,
	title={Collision Avoidance in Pedestrian-Rich Environments with Deep Reinforcement Learning},
	author={Michael Everett and Yu Fan Chen and Jonathan P. How},
	journal={arXiv preprint arXiv:1910.11689},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}

@article{Debard2019HCI,
	title={Learning 3D Navigation Protocols on Touch Interfaces with Cooperative Multi-Agent Reinforcement Learning},
	author={Quentin Debard an dJilles Steeve Dibangoye and St\'{e}phane Canu and  Christian Wolf},
	journal={arXiv preprint 	arXiv:1904.07802},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}


@article{Shi2019TNNLS,
	title={Multi Pseudo Q-Learning-Based Deterministic Policy Gradient for Tracking Control of Autonomous Underwater Vehicles},
	author={Wenjie Shi and Shiji Song and Cheng Wu and C. L. Philip Chen},
	journal={{IEEE} Transactions on Neural Networks and Learning Systems },
	volume={30},
	number={12},
	pages={3534 -- 3546},
	month={Dec.},
	year={2019},
	doi={10.1109/TNNLS.2018.2884797}
}

@article{Woo2019OE,
	title={Deep reinforcement learning-based controller for path following of an unmanned surface vehicle},
	author={Joohyun Woo and Chanwoo Yu and Nakwan Kim},
	journal={Ocean Engineering},
	volume={183},
	number={1},
	pages={155 -- 166},
	month={Dec.},
	year={2019},
	doi={10.1016/j.oceaneng.2019.04.099}
}


@article{Balachandar2019Soccer,
	title={Collaboration of AI Agents via Cooperative Multi-Agent Deep Reinforcement Learning},
	author={Niranjan Balachandar and Justin Dieter and Govardana Sachithanandam Ramachandran},
	journal={arXiv preprint arXiv:1907.00327},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}

@article{Anastassacos2019PartnerChoice,
	title={Understanding The Impact of Partner Choice on Cooperation and Social Norms by means of Multi-agent Reinforcement Learning},
	author={Nicolas Anastassacos and Steve Hailes and Mirco Musolesi},
	journal={arXiv preprint arXiv:1902.03185},
	volume={},
	number={},
	pages={},
	year={2019},
	doi={}
}



@article{Zhang2020TIM,
	title={Improved UDE and LSO for a Class of Uncertain Second-Order Nonlinear Systems Without Velocity Measurementss},
	author={Xinyu Zhang and Hui Li and Bo Zhu  and Yang Zhu},
	journal={{IEEE} Transactions on Instrumentation and Measurement },
	volume={69},
	number={7},
	pages={4076 -- 4092},
	month={Jul.},
	year={2020},
	doi={10.1109/TIM.2019.2942508}
}

@article{Zhang2020TCST,
	title={Optimization-Based Collision Avoidance},
	author={Xiaojing Zhang and Alexander Liniger  and Francesco Borrelli
	},
	journal={IEEE Transactions on Control Systems Technology},
	volume={},
	number={},
	pages={},
	month = {},
	year={2020},
	doi={10.1109/TCST.2019.2949540},
	note ={(Early Access)}
}


@article{Fan2020IJRR,
	title={Distributed multi-robot collision avoidance via deep reinforcement learning for navigation in complex scenarios},
	author={Tingxiang Fan and Pinxin Long and Wenxi Liu and Jia Pan},
	journal={The International Journal of Robotics Research},
	volume={39},
	number={7},
	pages={856?892},
	month = {May},
	year={2020},
	doi={10.1177/0278364920916531}
}


@article{Zhang2020MRRL_arXiv,
	title={Model-Reference Reinforcement Learning Control of Autonomous Surface Vehicles with Uncertainties},
	author={Qingrui Zhang and Wei Pan and Vasso Reppa},
	journal={arXiv preprint arXiv:2003.13839},
	volume={},
	number={},
	pages={},
	year={2020},
	doi={}
}

@book{royden1968real,
	title={Real analysis},
	author={Royden, Halsey Lawrence},
	year={1968},
	publisher={Krishna Prakashan Media}
}



%------------------------------------------------------------------------------
%    ---------------------------     Books     ---------------------------
%------------------------------------------------------------------------------

@Book{Ioannou1996,
	title     = {Robust Adaptive Control},
	publisher = {Prentice-Hall, Inc.},
	year      = {1996},
	author    = {Petros A. Ioannou and Jing Sun},
	edition   = {},
	comment   = {},
	timestamp = {},
}

@Book{Sutton2018MIT,
	title     = {Reinforcement Learning: An Introductions},
	publisher = {The MIT Press},
	year      = {2018},
	author    = {Richard S. Sutton and Andrew G. Barto},
	edition   = {2nd},
	comment   = {A very good book talks about some basic concepts in aerodynamics. It's very suitable for beginners.},
	timestamp = {2015.05.23},
}

@Book{Diestel2000Book,
	title     = {Graph Theory},
	publisher = {Springer-Verlag},
	year      = {2000},
	author    = {Reinhard Diestel},
	address   = {New York, NY, USA},
	edition   = {2nd Edition},
	comment   = {Very good introductory to many numerical topics. Definitely directed
		toward engineers.},
	timestamp = {2008.05.05},
}

@Book{Godsil2001Book,
	title     = {Algebraic Graph Theory},
	publisher = {Springer-Verlag},
	year      = {2000},
	author    = {Chris Godsil and Gordon Royle},
	address   = {New York, NY, USA},
	comment   = {Very good introductory to many numerical topics. Definitely directed
		toward engineers.},
	timestamp = {2008.05.05},
}

@BOOK{Khalil2002Book,
	title = {Nonlinear Systems},
	publisher = {Prentice Hall},
	year = {2001},
	author = {Hassan K. Khalil},
	edition = {3rd Edition},
	owner = {},
	review = {},
	timestamp = {2015.05.05}
}

@book{Dixon2003Book,
	Author = {Warren E. Dixon and Aman Behal and Darren M. Dawson and Siddharth P. Nagarkatti},
	Publisher = {Springer Science \& Business Media},
	Title = {Nonlinear Control of Engineering Systems: A Lyapunov-Based Approach},
	Year = {2003}
}

@book{Farrell2006Book,
	Author = {Jay A. Farrell and Marios M. Polycarpou},
	Publisher = {New York, NY: Wiley},
	Title = {Adaptive Approximation Based Control: Unifying Neural, Fuzzy and Traditional Adaptive Approximation Approaches},
	Year = {2006}
}




@book{Fossen2011Handbook,
	author    = "Thor I. Fossen",
	title     = "Handbook of Marine Craft Hydrodynamics and Motion Control",
	year      = "2011",
	publisher = "John Wiley \& Sons, Inc.",
	address   = "",
	doi ={}
}

@inbook{Majohr2006,
	author={J. Majohr  and  T. Buch},
	year= 2006, 
	chapter={Modelling, simulation and control of an autonomous surface marine vehicle for surveying applications Measuring Dolphin MESSIN}, 
	editor = {G.N. Roberts and R. Sutton }, 
	title= {Advances in Unmanned Marine Vehicles}, 
	publisher= {Institution of Engineering and Technology},
	address= {}, 
	doi = {10.1049/PBCE069E_ch16}
}

@inproceedings{sutton2009convergent,
	title={A convergent $ o (n) $ temporal-difference algorithm for off-policy learning with linear function approximation},
	author={Sutton, Richard S and Maei, Hamid R and Szepesv{\'a}ri, Csaba},
	booktitle={Advances in neural information processing systems},
	pages={1609--1616},
	year={2009}
}

@article{jiang2012computational,
	title={Computational adaptive optimal control for continuous-time linear systems with completely unknown dynamics},
	author={Jiang, Yu and Jiang, Zhong-Ping},
	journal={Automatica},
	volume={48},
	number={10},
	pages={2699--2704},
	year={2012},
	publisher={Elsevier}
}
@inproceedings{boukas2000robust,
	title={Robust stability and  \protect{$H_\infty$} control of discrete-time jump linear systems with time-delay: an \protect{LMI} approach},
	author={Boukas, EK and Liu, ZK},
	booktitle={Decision and Control, 2000. Proceedings of the 39th IEEE Conference on},
	volume={2},
	pages={1527--1532},
	year={2000},
	organization={IEEE}
}

@book{lyapunov1892general,
	title={The general problem of the stability of motion (in Russian)},
	author={Lyapunov, Aleksandr Mikhailovich},
	publisher={PhD Dissertation, Univ. Kharkov},
	year={1892}
}
@book{lewis2012optimal,
	title={Optimal control},
	author={Lewis, Frank L and Vrabie, Draguna and Syrmos, Vassilis L},
	year={2012},
	publisher={John Wiley \& Sons}
}

@inproceedings{petridis2006construction,
	title={Construction of neural network based \protect{\protect{Lyapunov}} functions},
	author={Petridis, Vassilios and Petridis, Stavros},
	booktitle={The 2006 IEEE International Joint Conference on Neural Network Proceedings},
	pages={5059--5065},
	year={2006},
	organization={IEEE}
}

@article{perkins2002lyapunov,
	title={\protect{Lyapunov} design for safe reinforcement learning},
	author={Perkins, Theodore J and Barto, Andrew G},
	journal={Journal of Machine Learning Research},
	volume={3},
	number={Dec},
	pages={803--832},
	year={2002}
}
@article{postoyan2017stability,
	title={Stability analysis of discrete-time infinite-horizon optimal control with discounted cost},
	author={Postoyan, Romain and Bu{\c{s}}oniu, Lucian and Ne{\v{s}}i{\'c}, Dragan and Daafouz, Jamal},
	journal={IEEE Transactions on Automatic Control},
	volume={62},
	number={6},
	pages={2736--2749},
	year={2017},
	publisher={IEEE}
}

@article{gorges2017relations,
	title={Relations between model predictive control and reinforcement learning},
	author={Gorges, Daniel},
	journal={IFAC-PapersOnLine},
	volume={50},
	number={1},
	pages={4920--4928},
	year={2017},
	publisher={Elsevier}
}

@mastersthesis{Castaneda2016MASc,
	author    = {Alvaro Ovalle Casta\~neda},
	title     = {Deep Reinforcement Learning Variants of Multi-Agent Learning Algorithms},
	school    = {University of Edinburgh},
	type     = {Master of Science},
	year      = {2016},
	note     = {}
}

@article{haarnoja2018soft,
	title={Soft actor-critic: Off-policy maximum entropy deep reinforcement learning with a stochastic actor},
	author={Haarnoja, Tuomas and Zhou, Aurick and Abbeel, Pieter and Levine, Sergey},
	journal={arXiv preprint arXiv:1801.01290},
	year={2018}
}

%------------------------------------------------------------------------------
%    ---------------------------     Report     ---------------------------
%------------------------------------------------------------------------------
@techreport{Garant2015Accel_MARL,
	title={Accelerating Multi-agent Reinforcement Learning with Dynamic Co-learning},
	author={Dan Garant and Bruno Castro da Silva and Victor Lesser and Chongjie Zhang},
	year={2015},
	institution={University of Massachusetts Amherst},
	url={http://mas.cs.umass.edu/paper/532},
	note={Technical Report UM-CS-2015-004}
}

@article{peters2019ergodicity,
	title={The ergodicity problem in economics},
	author={Peters, Ole},
	journal={Nature Physics},
	volume={15},
	number={12},
	pages={1216--1221},
	year={2019},
	publisher={Nature Publishing Group}
}

@article{moore2015ergodic,
	title={Ergodic theorem, ergodic theory, and statistical mechanics},
	author={Moore, Calvin C},
	journal={Proceedings of the National Academy of Sciences},
	volume={112},
	number={7},
	pages={1907--1911},
	year={2015},
	publisher={National Acad Sciences}
}

